Behavior Priors for Efficient Reinforcement Learning

As we deploy reinforcement learning agents to solve increasingly challenging problems, methods that allow us to inject prior knowledge about the structure of the world and effective solution strategies becomes increasingly important. In this work we consider how information and architectural constraints can be combined with ideas from the probabilistic modeling literature to learn behavior priors that capture the common movement and interaction patterns that are shared across a set of related tasks or contexts. For example the day-to day behavior of humans comprises distinctive locomotion and manipulation patterns that recur across many different situations and goals. We discuss how such behavior patterns can be captured using probabilistic trajectory models and how these can be integrated effectively into reinforcement learning schemes, e.g.\ to facilitate multi-task and transfer learning. We then extend these ideas to latent variable models and consider a formulation to learn hierarchical priors that capture different aspects of the behavior in reusable modules. We discuss how such latent variable formulations connect to related work on hierarchical reinforcement learning (HRL) and mutual information and curiosity based objectives, thereby offering an alternative perspective on existing ideas. We demonstrate the effectiveness of our framework by applying it to a range of simulated continuous control domains.

==> older_version/background.tex <==
\section{Background}
\label{sec:background}
We now introduce some notation and background information that we will serve as the basis of the work in later sections.

\subsection{Reinforcement Learning and MDPs}
\label{sec:RL}
We start with some the background definitions for RL and Markov decision processes (MDPs) \citep{suttonbarto}. In the following we will limit discussion to the infinite-horizon discounted setting for simplicity.
A Markov Decision Process (MDP) is defined by the following: $S$ and $A$ are state and action spaces, with $P: S \times A \times S \rightarrow \mathbb{R}_{+}$ a state-transition probability function or system dynamics and
$P_0: S \rightarrow \mathbb{R}_{+}$ an initial state distribution. We denote trajectories by $\tau = (s_0, a_0, s_1, a_1, \dots)$ and the state-action history at time step $t$ including $s_t$ (but not $a_t$) with $x_t = (s_0, a_0, \dots s_t)$.
%
We consider policies $\pi$ that are \emph{history-conditional} distributions over actions $\pi(a_t|x_t)$ \footnote{
%We generally work with history dependent policies since even in MDPs regularization and / or restricted access to state information may render the setup effectively partially observed.
We generally work with history dependent policies since we will consider restricting access to state information from policies (for information asymmetry), which may render fully observed MDPs effectively partially observed.
}. The learning objective is to maximise expected discounted returns, given by a reward function $R: S \times A \rightarrow \mathbb{R}$, and a discount factor $\gamma\in [0,1)$. 

Given the initial state distribution, transition dynamics and policy, the joint distribution over trajectories $\tau$ is given as:
\begin{align}
\pi(\tau) = 
    P_0(s_0)\pi(a_0|x_0)\prod_{t=1}^T P(s_t|s_{t-1},a_{t-1})\pi(a_t|x_t).
\end{align}
where $s_t\in S$ is the state at time $t\ge 0$ and $a_t\in A$ the corresponding action. 
For notational convenience, we have overloaded $\pi$ here to represent both the policy as well as the distribution over trajectories.
%
Given a trajectory $\tau$, the discounted return is
\begin{align}
    R(\tau) = \sum_{t=0}^\infty \gamma^t R(s_t,a_t)
\end{align}
The expected discounted returns over trajectories is then
\begin{align}
\mathcal{J}(\pi) = \EE_{\pi}[R(\tau)],
\end{align}
where the expectation is with respect to the trajectory distribution defined above. The goal of RL methods is to find an optimal policy $\pi^*(a | x)$ that maximizes the expected discounted return $\mathcal{J}(\pi)$ \citep{suttonbarto}.

Given a policy, the value functions $V^\pi(x)$ (and $Q^\pi(x,a)$) are the expected discounted returns when starting in state $x$ (and action $a$):
\begin{align}
V^\pi(x_t) &= \EE_{\pi}[R(\tau)|x_t]
= \EE_{\pi(a|x_t)}[Q^\pi(x_t,a)] \nonumber \\
Q^\pi(x_t,a_t) &= \EE_{\pi}[R(\tau)|x_t,a_t]
= R(s_t,a_t) + \gamma \EE_{P(s_{t+1}|s_t,a_t)}[V^\pi(x_{t+1})].
\end{align}

% \subsection{Overview of probabilistic modeling}
% \label{sec:ELBO}

% \def\param{\theta}
% \def\model{p_\param}
% \def\varpost{q}
% \def\varparam{\phi}
% \def\latent{z}
% \def\data{x}
% \def\all{{1:N}}

% \dhruva{Remove this bit.}
% We briefly revisit core ideas in probabilistic machine learning to provide background for their use in the rest of the paper. We refer the reader to \cite{bishop2006pattern,koller2009probabilistic,murphy2012machine} for introductory textbooks on probabilistic learning. 

% Assume we are given a dataset $\data_\all = \{ \data_1, \dots \data_N \}$. Probabilistic learning is framed in the context of a \emph{generative model} $\model$, which is a joint distribution of the data parameterised by $\param$, potentially involving latent variables which we denote as $\latent$, and potentially including contextual information or covariates. For simplicity, though the framework is more general, we will assume that the data is \emph{independent and identically distributed (iid)} under the model, i.e.\, 
% \begin{align}
% \model(\data_\all) = \prod_{i=1}^N \model(\data_i)
% = \prod_{i=1}^N \int \model(\data_i|\latent_i)\model(\latent_i) d\latent_i
% \end{align}
% where we have also introduced one iid latent variable $\latent_i$ corresponding to each observed datum $\data_i$. For intuition, each datum can be an image while the latent variable describes the unobserved properties of the visual scene. $\model(z)$ is a prior distribution, e.g.\ over visual scenes, and $\model(x|z)$ is an observation model, e.g.\ of the image given the scene.

% In this framework, \emph{inference} refers to computation or approximation of the posterior distribution over latent variables given observed data given by Bayes' rule, i.e.,\ 
% \begin{align}
% \model(\latent|\data)
% = \frac{\model(\data|\latent)\model(\latent)}{\model(\data)}
% = \frac{\model(\data|\latent)\model(\latent)}{\int \model(\data|\latent)\model(\latent)d\latent}
% \end{align}
% while \emph{learning} refers to estimation of the model parameters $\param$ from data. Typically this is achieved by maximising the log \emph{likelihood}, i.e.\ the log marginal probability of the data as a function of the parameters $\param$:
% \begin{align}
%     \param^\text{MLE} = \arg\max_\param \log \model(\data_\all)
%     = \arg\max_\param \sum_{i=1}^N \log \model(\data_i) \label{eq:mle}
% \end{align} 

% The core difficulty of the probabilistic learning framework is in the computation of the log marginal and posterior probabilities (as well as their gradients).  These are intractable to compute exactly for most models of 

% A common approach is to employ a variational approximation. This stems from the following lower bound on the log marginal probability obtained by applying Jensen's inequality. For any conditional distribution $\varpost(\latent|\data)$ and any $x$, we have:
% \begin{align}
%     \log \model(\data) &= \log \int \model(\data, \latent) d\latent = \log \int \varpost(\latent|\data)\frac{\model(\data, \latent)}{\varpost(\latent|\data)} d \latent \label{eq:log-marginal}\\
%     &= \log \EE_\varpost \left [ \frac{\model(\data, \latent)}{\varpost(\latent|\data)} \right ]
%     \geq \EE_\varpost\left[ \log \frac{\model(\data,\latent)}{\varpost(\latent|\data)} \right]
%     \label{eq:elbo-1}\\
%     &= \EE_\varpost\left[\log \model(\data|\latent) + \log\frac{\model(\latent)}{\varpost(\latent|\data)}\right]  
%     =  \EE_\varpost\left[\log \model(\data|\latent)\right] - \KL [ \varpost(\latent|\data) || \model(\latent) ]
%     \label{eq:elbo-2}\\
%     &= \EE_\varpost\left [  \log \model(\data) + \log \frac{\model(\latent|\data)}{\varpost(\latent|\data)} \right ] 
%     =  \log \model(\data) - \KL [ \varpost(\latent|\data) || \model(\latent | \data) ],
%     \label{eq:elbo-3}
% \end{align}
% where we use Jensen's inequality for lower bound in \eqref{eq:elbo-1}.  \eqref{eq:elbo-2} and \eqref{eq:elbo-3} show two equivalent ways of writing the resulting bound, the first of which is tractable and the second of which is intractable but gives a different way to see that the expression gives a lower bound on the log marginal probability, since the KL divergence is non-negative.
% %
% This bound is often referred to as evidence lower bound or \emph{ELBO}. As the last line shows the bound is tight when $\varpost$ matches the true posterior $\model(\latent | \data)$. For most models the true posterior is as intractable as the log marginal probability\footnote{This is not surprising considering that $\model(\latent | \data) = \model(\data,\latent) / \model(\data)$, i.e.\ the normalization constant of the posterior is exactly the intractable marginal probability.} and $\varpost$ is thus chosen to belong to some restricted family parameterised by variational parameters $\varparam$.

% Plugging this lower bound into \eqref{eq:mle}, we get the following objective to be maximized with respect to model parameters $\param$ and variational parameters $\varparam$:
% \begin{align}
%     \sum_{i=1}^N \log \model(\data_i)
%     \ge \sum_{i=1}^N
%     \EE_{\varpost_\varparam(\latent_i|\data_i)}\left[
%     \log\model(\data_i|\latent_i) + \log\model(\latent_i) - \log\varpost_\varparam(\latent_i|\data_i)\right] \label{eq:elbo:objective}
% \end{align}

==> older_version/bp_experiments.tex <==
\section{Experiments}
\label{sec:experiments}
In this section, we demonstrate the advantage of \bps experimentally on a number of simulated continuous control domains using walkers from the DeepMind control suite \citep{tassa2018control} developed using the MuJoCo simulation framework \citep{todorov2012mujoco}. 

The remainder of this section is split into two parts. In the first part, we develop the intuition for these \textit{priors} further through the use of a simple toy-like domain where we analyze how various architectures can be used to model the structure in a task at different levels of complexity. Secondly, we run a set of ablation experiments to study the importance of information asymmetry to our approach. We leave further experiments showing the advantage of \bps for learning and transfer across a range of tasks to Section \ref{sec:hier_experiments}. 

All of the tasks we consider in this work use sparse rewards.
Unless otherwise specified, learning curves show returns (on the Y-axis) as a function of the number of environment steps processed by the learner (X-axis) and for each curve, we plot the best performing configuration averaged across 5 seeds. A complete list of hyperparameters swept over is included in Appendix \ref{appendix:experiment_details}. We run all experiments with a distributed setup using a replay buffer with 32 actors and 1 learner. 
% \dhruva{TODO: Ref for replay buffer}
\subsection{Note on Tasks}
In this section and section \ref{sec:hier_experiments}, we conduct experiments over a wide range of tasks that vary in terms of the complexity of the task itself and the body used as shown in figure \ref{fig:task_bodies}. All of the tasks that we consider involve learning specific behaviors to achieve one or many sub-goals. For brevity, we name the tasks according the sub-goals associated with them.
%For brevity, we have given short-form names for these tasks that describe the \texit{behaviors} required to solve them. 
Specifically, these could involve simply going to a specified target location, which we will refer to as 'Locomotion' or they might involve moving boxes to target locations which we will refer to as 'Manipulation'. We vary the complexity of the tasks using - more complicated bodies (\textit{Locomotion (Humanoid)}); varying the number of boxes or targets (\textit{Manipulation (2 boxes, 2 targets)}); or by combining them (\textit{Locomotion and Manipulation}). For convenience, we have summarized the tasks used in this section and section \ref{sec:hier_experiments} (demarcated with a *) in Table \ref{table:task_list}. A more complete description is available in Appendix \ref{appendix:tasks}. The only exception to this nomenclature are the toy experiments described in section \ref{sec:toy_domain_1}. 

\begin{figure}%
    \centering
    \subfloat[All bodies considered. \label{fig:bodies}]{{\includegraphics[height=2.5cm]{figures/Bodies.png} }}%
    \qquad
    \subfloat[Some of the tasks considered \label{fig:tasks}]{{\includegraphics[height=2.5cm]{figures/tasks.png} }}%
    \caption{\textbf{Visualization of tasks and bodies.} An illustration of some of the tasks and the bodies used for our experiments.}
    \label{fig:task_bodies}
\end{figure}


\subsection{Toy Domain: Pointmass on Grid}
\label{sec:toy_domain_1}
In order to develop an intuition for our method we first consider a toy domain where a 2-dof (degree of freedom) pointmass must learn to visit 4 targets in some sequence on a 2D plane as illustrated by figure \ref{fig:visualize_traj}. The agent action is fed as torque input to move the body along the x and y-axes. The target locations are randomized at the start of each episode and the agent is given a reward of +10 each time it visits the correct target in the sequence.
We consider two versions of this task:
% as shown in Figure \ref{fig:pretraining}. 
\begin{itemize}
    \item \textbf{Easy Task}: The agent is given the immediate next target to visit as input at each point in time.
    \item \textbf{Hard Task}: The agent is must visit the 4 targets in sequence (target 1 followed by target 2 and so on..) and does not receive any additional information. In this version, the agent receives a bonus reward of +50 for completing the task. 
\end{itemize}

In both variants of the task, the agent receives the coordinates of all of the targets as well as its own location and velocity information. The \bps also receive this information but do not get the task specific information described above. %As we will show, the resulting information asymmetry between the \textit{prior} and the policy  and also allows for a prior trained on one task to be transferred to the other. 

We introduce another layer of complexity to the task by adding structure to the way the targets are chosen. Specifically, the sequence of targets is chosen based on 2nd order Markovian dynamics where some targets are more likely to be chosen given the last two targets that were visited. (see appendix \ref{appendix:environments} for more details)%While this choice may seem somewhat arbitrary, 
As we will show, this allows us to gain insight into how different architectures allow us to model structure at various levels.

Specifically, we consider two architectures for our \bps - one that only has an MLP and another that incorporates an LSTM \citep{lstm} architecture and can thus learn longer term temporal correlations. In both cases the policy and critic include LSTMs. 

\begin{figure}%
    \centering
    \subfloat[Exploration with a randomly initialized Gaussian policy. \label{fig:visualize_random}]{{\includegraphics[height=4cm]{figures/set_1/pointmass_gaussian_exploration.png} }}%
    \qquad
    \subfloat[Exploration with the learnt \bp model (LSTM). \label{fig:visualize_prior}]{{\includegraphics[height=4cm]{figures/set_1/pointmass_prior_exploration.png} }}%
    \caption{\textbf{Visualization of exploration using a \bp}. Each colored dotted line represents a trajectory generated by rolling out a policy in the task.}
    \label{fig:visualize_traj}
\end{figure}

\begin{figure}%
    \centering
    \subfloat[Learning with priors on Easy Task\label{fig:easy_set_1}]{{\includegraphics[width=0.45\linewidth]{figures/set_1/easy_task_set_1.png} }}%
    \qquad
    \subfloat[Transfer of priors to hard task\label{fig:hard_set_1}]{{\includegraphics[width=0.45\linewidth]{figures/set_1/transfer_hard_task_set_1.png} }}%
    \caption{\textbf{Learning and transfer on toy domain.} Learning curves from training on the easy task and transferring to the hard task with various \bp architectures.}
    \label{fig:pointmass_results}
\end{figure}

Figure \ref{fig:pointmass_results} shows the result of training and transfer using different \bp models on this domain. As shown in Figure \ref{fig:easy_set_1}, using either the LSTM or MLP prior \textbf{boosts learning performance} on the easy task. We found no significant difference between the two types of priors during learning. 

In Figure \ref{fig:hard_set_1} we transfer the \bp trained on the easy task to the hard task. Since there is no additional information to the agent beyond what the \textit{prior} receives, we use the \textit{prior} to initialize the weights of the agent policy as well in this case. 
% We ran this experiment with fewer actors per learner (4) which favors methods that are more data efficient. 
Each training curve averages across 10 seeds (2 seeds for each of the 5 seeds from training). 
% We observe that in this setup, this task \textit{cannot} be learned without the use of a \bp.
We find the LSTM model performs significantly better than the MLP in this case since it can better capture the temporal structure present in the task. Specifically, the target sequence for transfer is \textit{more likely} to be generated under the Markovian dynamics introduced during pretraining. Therefore a model that fits more closely to that space of trajectories has an advantage during transfer. We analyze this in greater detail below.

\subsubsection{Analysis}

In figure \ref{fig:visualize_traj} we illustrate the structure captured by the \textit{priors} and demonstrate why they are useful for transfer. As shown in figure \ref{fig:visualize_prior}, trajectories generated by rolling out the learnt prior result in more "goal-directed" behavior where the agent is far more likely to visit the targets. This is in stark contrast to the exploration of a randomly initialized Gaussian policy as shown in figure \ref{fig:visualize_random}. Since the \bp does not have access to the task information pertaining to \textit{which specific target} to visit next, it instead learns to encode the behavior of visiting targets in general. 


In figure \ref{fig:transition_dynamics}, we plot the probability of visiting target 0 against the last 2 visited targets for the different \bp models. As opposed to the MLP prior that visits each target more or less uniformly, the LSTM architecture learns to capture the underlying transition dynamics of the domain. This in turn results in a significant boost in performance during transfer where the agent is more likely to see the rewarding sequence.
%and thus learns to capture the additional structure 
% of the domain. In contrast, the MLP prior visits each target more or less uniformly. 

% Therefore the \textbf{choice} of \bp model plays an important role in the space of trajectories that the prior learns to capture. 
It is important to note that restricting the space of trajectories that the prior explores is only advantageous if that space also captures the \textit{solution space} of the task we are ultimately interested in solving. In other words, there is a tradeoff between generality and efficacy of the prior. A prior over trajectories that is 'uniform' in that it assigns equal mass to \emph{all possible trajectories} may actually be of limited use since it does not capture any of the underlying \textit{task structure}.
%may be too spread out to be of much use.
% \dhruva{Should we mention this here? It would be more easily digested with the negative transfer task perhaps. In general perhaps we should consider a negative transfer result as well?}

\begin{figure}%
    \centering
    \includegraphics[width=\linewidth, height=6cm]{figures/set_1/transition_dynamics_set_1.png}
    \caption{\textbf{Transition dynamics} generated under different \bp models to visit target 0. Each point on the x-axis indicates the indices of the last two targets visited. On the y-axis we plot the probability of visiting target 0 for each transition sequence.}
    \label{fig:transition_dynamics}
    % \begin{subfigure}{0.5\textwidth}
    % \centering
\end{figure}

\begin{table}[htp]
\centering
\begin{tabular}{ | m{2.3cm} | m{2.5cm}| m{1.6cm} |  m{1.2cm} |  m{2cm} | m{2cm} |} 
 \hline
 \textbf{Task Name} & \textbf{Description} & \textbf{Body} & \textbf{Action Dim.} & \textbf{Obs.} & \textbf{Obs. to \textit{Prior}} \\
 \hline\hline
  \hline
 
 \textit{Locomotion (Humanoid)} & Follow a moving target  & Humanoid & 23 & Proprio +
  Target location & Varies (See text) \\ 
 
 \hline
 
 \textit{Locomotion (Ant)} & Go to one of 3 targets  & Ant & 8 & Proprio + Targets + Index of goal & Varies (See text) \\ 

 \hline
 
 \textit{Locomotion (Gaps)*} & Move forward and jump across a variable length gap. & Ant & 8 & Proprio + Global position + Gap length & Proprio \\ 

 \hline
 
 \textit{Locomotion and Manipulation} & Move a box to a specified target and then move to another target.  & Ant & 8 & Proprio + Box + Targets + Task encoding & Varies (See text) \\ 
 
 \hline
 
 \textit{Manipulation (1 box, 1 target)*} & Move a box to a target location.  & Ant & 8 & Proprio + Box + Targets + Task encoding & Proprio + Box \\
 
 \hline
 
 \textit{Manipulation (1 box, 3 target)*} & Move a box to one of 3 target locations.  & Ant & 8 & Proprio + Box + Targets + Task encoding & Proprio + Box \\ 
 
 \hline
 
 \textit{Manipulation (2 box, 2 target)*} & Move one of two boxes to one of 2 target locations.  & Ball & 2 & Proprio + Boxes + Targets + Task encoding & Proprio + Boxes \\ 
 
 \hline
 
 \textit{Manipulation (2 box gather)*} & Move two boxes close together.  & Ball & 2 & Proprio + Boxes + Targets + Task encoding & Proprio + Boxes \\ 
 \hline
 
\end{tabular}
\caption{\textbf{List of Tasks} A short summary of tasks used along with the information asymmetry used to train the \bp. Tasks marked with a '*' are considered in section \ref{sec:hier_experiments}. A more complete description is presented in Appendix \ref{appendix:tasks}.}
\label{table:task_list}
\end{table}

% Experiments on the flat priors.
\subsection{Effect of Information Asymmetry}

\subsubsection{Locomotion and Manipulation Task}
\label{sec:info_asym_1}
In this section we demonstrate empirically the importance of information asymmetry in learning \bps. We focus the discussion on the complex \textit{Locomotion and Manipulation} task. In this task, the agent must move to a certain goal location (locomotion) and also move a box to another target location (manipulation). The agent receives a reward of +10 for successfully accomplishing either sub-task and an added bonus  of +50 when it solves both. 
For this task we use an 8-DoF ant walker as shown in Figure \ref{fig:task_bodies}.

Apart from the proprioceptive information that contains the relative joint positions and velocities of the agent's body (refer to Appendix \ref{appendix:bodies}), the agent also gets the location of the targets, the box and a one-hot encoding indicating which target it must push the box to. There are therefore many choices of subsets of information that can be sent to the \textit{prior}. For this task we used additional encoding networks for each input sub-component as we found this sped up learning (more details in Appendix \ref{appendix:experiment_details}).

\begin{figure}%
    \centering
    \includegraphics[width=\linewidth]{figures/set_1/info_asym_mbgtt.png}
    \caption{\textbf{Effect of information asymmetry.} Effect of learning with different levels of information asymmetry on the \textit{Locomotion and Manipulation} task.}
    \label{fig:info_asym_mbgtt}
    % \begin{subfigure}{0.5\textwidth}
    % \centering
\end{figure}

We experiment with various settings of information asymmetry between the \bp and the agent policy in figure \ref{fig:info_asym_mbgtt}. On this task we find a marked difference in performance based on the information that the \bp has access to. We observe that most policies (including training from scratch) can easily get stuck in a local minima wherein the agent learns to solve the easier locomotion component of the task but never learns about the additional reward for moving the box. However, as we see, certain \bps can help regularize against this sub-optimal behavior by encouraging useful patterns of behavior. For instance, a prior that has access to \textit{only} proprioceptive information would ostensibly encode the space of trajectories containing primitive gaits or movements.
%relating to the agent moving around in the environment. 
By encouraging the policy to continue to explore in this space, the agent is more likely to continue learning and to see the full task reward. In this case we find that the \bp that has access to both proprioception as well as the location of the box learns the fastest. We hypothesize that this prior could model the space of trajectories related to moving a box around which would be useful to get out of the local optima described above.

\subsubsection{Other Tasks}
\begin{figure}%
    \centering
    \includegraphics[width=\linewidth]{figures/set_1/info_asym_rest.png}
    \caption{\textbf{Effect of information asymmetry.} Effect of learning with different levels of information asymmetry on \textit{Manipulation (1 box, 3 targets)}, \textit{Locomotion (Humanoid)} and \textit{Locomotion (Ant)}.}
    \label{fig:info_asym_rest}
    % \begin{subfigure}{0.5\textwidth}
    % \centering
\end{figure}

In this section, we demonstrate the effect of information asymmetry for learning \bps on three tasks: \textit{Manipulation (1 box, 3 targets)}, \textit{Locomotion (Humanoid)} and \textit{Locomotion (Ant)} (refer to table \ref{table:task_list} for a short summary).
% \begin{itemize}
%     \item \textbf{Manipulate many (Ant)}: The ant must move a box to one of 3 target locations.
%     \item \textbf{Locomotion (Humanoid)}: This is a goal following task with the Humanoid body. The agent is given a goal location that it must reach, at which point a new goal is generated. This continue until the episode times out.
%     \item \textbf{Locomotion (Ant)}: The ant must move to one of 3 target locations.
% \end{itemize}

% The tasks were chosen to cover a range of complexities related to the task and agent body. 
We show our findings in Figure \ref{fig:info_asym_rest}.
We observe that regularizing against a \bp \textbf{always provides a benefit} and \textit{priors} with partial information always performs better than ones with full information. Additionally, \bps with access to only proprioceptive information tend to perform the best in tasks involving just locomotion. This is consistent with the intuition described earlier that this allows for priors that model general trajectory spaces that contain primitive movement patterns. 

Figure \ref{fig:gtt_humanoid} illustrates this point elegantly. In figure \ref{fig:gtt_humanoid_targets}, we show the trajectory followed by the humanoid in the \textit{Locomotion (Humanoid)} task where the target moves when the agent reaches it. In figure \ref{fig:gtt_humanoid_kl} we plot the KL divergence between the policy and the \bp where the \bp here only gets proprioceptive information. As the figure illustrates, the \bp and the policy match quite closely (and so the KL is low) until the agent reaches a target. At this point, the policy changes to a new pattern of movement in order to change direction and go toward the new target location. We observe spikes in the KL divergence precisely when new targets are spawned. These eventually reduce as the \bp adapts to the new movement pattern (after completing a turn say), indicating that the prior does indeed encode movements.

\begin{figure}%
    \centering
    \subfloat[Trajectory of humanoid visiting targets in the \textit{Locomotion (Humanoid)} task. \label{fig:gtt_humanoid_targets}]{{\includegraphics[width=0.45\linewidth]{figures/set_1/gtt_humanoid_targets.png} }}%
    \qquad
    \subfloat[Deviation of policy from the \bp in terms of KL divergence. \label{fig:gtt_humanoid_kl}]{{\includegraphics[width=0.45\linewidth]{figures/set_1/gtt_humanoid_kl.png} }}%
    \caption{\textbf{Analysis of the \textit{Locomotion (Humanoid)} task}. The spikes in KL divergence on the right align with the change in target as on the left; this is consistent with the idea that the \bp encodes primitive movement patterns.}
    \label{fig:gtt_humanoid}
\end{figure}

==> older_version/bp_experiments_v2.tex <==
\section{Experiments}
% Notes:
% Expand on intuition for tasks: 
%  why sparse reward; 
%  why locomotion; manipulation etc? - connect to prev section in terms of humanoid.
%  for pointmass- why do we want this structure?

\label{sec:experiments}
In this section, we analyze the effect of \bps experimentally on a number of simulated motor control domains using walkers from the DeepMind control suite \citep{tassa2018control} developed using the MuJoCo simulation framework \citep{todorov2012mujoco}. 
%
The purpose of these experiments is to understand how \textit{priors} with various capacity and information constraints can learn to capture general task-agnostic behaviors at different levels of abstraction, including both basic low-level motor skills as well as goal-directed and other temporally extended behavior.
With this in mind, we consider a range of multi-task and transfer problems where the solution space shares some common underlying structure which we can model at varying levels of detail and generality. 

%For instance, as described earlier, we consider a range of 'Locomotion' tasks all of which require a simulated agent to reach various goal locations. A common element underpinning these tasks is that the gait or underlying pattern of movement of any agent that solves is largely goal independent. In a similar vein, we consider a range of 'Manipulation' tasks which involve interacting with and moving objects to goals. 
%As described earlier, we consider a range of 'Locomotion' tasks all of which 
Our range of 'Locomotion' tasks
requires a simulated agent to reach various goal locations or manipulate objects in its environment.
The \emph{underlying structure} in all of these are the patterns of interaction between the agent and environment that are consistent across the solutions to each task. For instance, a common element underpinning these tasks is that the gait or underlying pattern of movement of any agent that solves it is largely goal independent. More specific and less general behavior that recurs across tasks includes goal-directed locomotion or object interactions. 
We further include problems that are specifically designed to exhibit structure at different temporal scales: In the 'Sequential Navigation' tasks an agent must visit several targets in \emph{sequence}, with some target sequences being much more likely than others. %which we define to be history dependent. 
In this setting we analyze how the prior model's architecture %different modeling constraints on the \textit{prior} 
affects the types of behavior that can be modeled. 

We vary the complexity of these tasks using more complicated bodies (\textit{Locomotion (Humanoid)}); changing the number of boxes or targets (\textit{Manipulation (2 boxes, 2 targets)}); or by combining them (\textit{Locomotion and Manipulation}).
All of the tasks that we consider in this work use sparse rewards. Sparse reward tasks are typically harder to learn from but are easier to specify since they do not require hand engineered per-timestep rewards. This setting provides an interesting context in which to study \bps. As the \textit{prior} learns to model solutions for some tasks, it can help \emph{shape} the learning process and guide the policy to discover solutions to new tasks. As we show below, this can lead to faster convergence for the policy on a range of tasks.

% As described in section \ref{sec:BP}, the \textit{prior} can be viewed as a shaping reward that can help guide the policy to solutions to more tasks. We therefore expect our method to be most beneficial in a 'sparse reward' setting and all the tasks we consider in this work thus use sparse rewards. 

%The only exception to this nomenclature are the toy experiments described in section \ref{sec:toy_domain_1}.
% The remainder of this section is split into two parts. In the first part, we develop the intuition for these \textit{priors} further through the use of a simple toy-like domain where we analyze how various architectures can be used to model the structure in a task at different levels of complexity. Secondly, we run a set of ablation experiments to study the importance of information asymmetry to our approach. We leave further experiments showing the advantage of \bps for learning and transfer across a range of tasks to Section \ref{sec:hier_experiments}. 
% Additionally, all of the tasks we consider in this work use sparse rewards. This helps illustrate an important aspect of jointly optimizing the \textit{prior} and policy in our approach. Similar to the observations of  \citet{teh2017distral}, as the prior learns a more general space of behaviors it can guide the policy to learn new tasks. For instance - 

For convenience, we have summarized the tasks used in this section and section \ref{sec:hier_experiments} (demarcated with a *) in Table \ref{table:task_list}. A more complete description is available in Appendix \ref{appendix:tasks}. 

Unless otherwise specified, learning curves show returns (on the Y-axis) as a function of the number of environment steps processed by the learner (X-axis) and for each curve, we plot the best performing configuration averaged across 5 seeds. A complete list of hyperparameters swept over is included in Appendix \ref{appendix:experiment_details}. We run all experiments with a distributed setup using a replay buffer with 32 actors and 1 learner. 
% \dhruva{TODO: Ref for replay buffer}
% \subsection{Note on Tasks}
% In this section and section \ref{sec:hier_experiments}, we conduct experiments over a wide range of tasks that vary in terms of the complexity of the task itself and the body used as shown in figure \ref{fig:task_bodies}. All of the tasks that we consider involve learning specific behaviors to achieve one or many sub-goals. For brevity, we name the tasks according the sub-goals associated with them.
%For brevity, we have given short-form names for these tasks that describe the \texit{behaviors} required to solve them. 
% Specifically, these could involve simply going to a specified target location, which we will refer to as 'Locomotion' or they might involve moving boxes to target locations which we will refer to as 'Manipulation'.  

\begin{figure}%
    \centering
    \subfloat[All bodies considered. \label{fig:bodies}]{{\includegraphics[height=2.5cm]{figures/Bodies.png} }}%
    \qquad
    \subfloat[Some of the tasks considered \label{fig:tasks}]{{\includegraphics[height=2.5cm]{figures/tasks.png} }}%
    \caption{\textbf{Visualization of tasks and bodies.} An illustration of some of the tasks and the bodies used for our experiments.}
    \label{fig:task_bodies}
\end{figure}


% \subsection{Toy Domain: Pointmass on Grid}
\subsection{Case study: Sequential Navigation}
\label{sec:toy_domain_1}
% 1. Develop intuition 'history-dependent' structure.
% 2. Modeling constraints in terms of MLP/LSTM.
% 3. Overall note- descriptions can be more concise.
We begin our analysis on a range of 'Sequential Navigation' tasks where an agent must learn to visit targets in some sequence as illustrated by figure \ref{fig:visualize_traj}. The goal of this set of experiments is to analyze how %different modeling constraints 
model capacity (i.e. model architecture)
can affect the \emph{kinds of behaviors} that are captured by a \bp. To this end, %we introduce a layer of complexity to this task by incorporating temporally correlated structure in the way the sequence to visit is chosen. 
%Specifically, each new target is chosen based on 2nd order Markovian dynamics where some targets are more likely to be chosen given the last two targets that were visited (see appendix \ref{appendix:environments} for more details).
we study tasks are designed to exhibit structure at multiple temporal and spatial scales. Specifically, sequences of targets are chosen based on 2nd order Markovian dynamics where some targets are more likely to be chosen given the two preceding targets than others (see appendix \ref{appendix:environments} for more details). In this setting the behavioral structure that could usefully be modeled by the behavior prior includes, effectively, a hierarchy of behaviors of increasing specificity: undirected locomotion behavior, goal-directed locomotion, as well as the long-horizon behavior that arises from some target sequences being more likely than others.



% Adding this structure to the task enables us to analyze how different modeling constraints can affect the kinds of behaviors captured by the \bp.
To complement the structure in the task, we consider two kinds of models for our \bps - one that only uses a Multi-layer perceptron (MLP) architecture and another that incorporates an LSTM \citep{lstm} and can thus learn to model temporal correlations. In both cases the policy and critic include LSTMs. Our goal is to analyze the kinds of behaviors each of these models can learn and understand the effect this has on learning and transfer.

With this in mind, we consider two versions of this task:
\begin{itemize}
    \item \textbf{Sequential Navigation Easy}: In this setting the agent is given the immediate next target to visit as input at each point in time.
    \item \textbf{Sequential Navigation Hard}: Here, the agent must visit 4 targets in sequence (target 1 followed by target 2 and so on..) and does not receive any additional information. Crucially, the sequence of targets used during transfer is \emph{more likely} to be generated under the Markovian dynamics used for training (compared to a uniform distribution over 4 target sequences). In this version, the agent receives a bonus reward of +50 for completing the task. 
\end{itemize}

In both variants of the task, the agent receives the coordinates of all of the targets as well as its own location and velocity information. The \bps also receive this information but \emph{do not get the task specific information} described above. To begin with, we consider a version of this task with the 2-dof pointmass body. The target locations are randomized at the start of each episode and the agent is given a reward of +10 each time it visits the correct target in the sequence.

\begin{figure}[t]
    \centering
    \subfloat[Exploration with a randomly initialized Gaussian policy. \label{fig:visualize_random}]{{\includegraphics[width=0.3\linewidth]{figures/set_1/pointmass_gaussian_exploration.png} }}%
    \qquad
    \subfloat[Exploration with the learnt \bp model (LSTM). \label{fig:visualize_prior}]{{\includegraphics[width=0.3\linewidth]{figures/set_1/pointmass_prior_exploration.png} }}%
    \caption{\textbf{Visualization of exploration using a \bp}. Each colored dotted line represents a trajectory generated by rolling out a policy in the task.}
    \label{fig:visualize_traj}
\end{figure}

% width=0.45\linewidth
\begin{figure}%
    \centering
    \subfloat[Learning with priors on Easy Task\label{fig:easy_set_1}]{{\includegraphics[scale=0.28]{figures/set_1/easy_task_set_1.png} }}%
    \qquad
    \subfloat[Transfer of priors to hard
    task\label{fig:hard_set_1}]{{\includegraphics[scale=0.28]{figures/set_1/hard_task_set_1.png} }}%
    \caption{\textbf{Learning and transfer on Sequential Navigation.} Learning curves from training on the easy task and transferring to the hard task with various \bp architectures.}
    \label{fig:pointmass_results}
\end{figure}

We illustrate our results in figure \ref{fig:pointmass_results}. 
Figure \ref{fig:easy_set_1} shows that learning with \textit{either prior} leads to faster convergence on this task. This is in line with our intuition that the \textit{structure} captured by the \textit{prior} can guide the learning process. These behaviors are also useful to learn the transfer task as shown in figure \ref{fig:hard_set_1}. For this task, since there is no additional information to the agent beyond what the \textit{prior} receives, we use the \textit{prior} to initialize the weights of the agent policy as well in this case. However since we do not transfer the critic and the SVG-0 algorithm relies on an informed critic to guide policy learning, we see a drop in performance across all curves to begin with.
Each training curve for transfer averages across 10 seeds (2 seeds for each of the 5 seeds from training). 
% Figure \ref{fig:pointmass_results} shows the result of training and transfer using different \bp models on this domain. As shown in Figure \ref{fig:easy_set_1}, using either the LSTM or MLP prior \textbf{boosts learning speed} on the easy task. We found no significant difference between the two types of priors during learning. 
% We ran this experiment with fewer actors per learner (4) which favors methods that are more data efficient. 
% We observe that in this setup, this task \textit{cannot} be learned without the use of a \bp.
We find the LSTM model performs significantly better than the MLP during transfer. As expected, the constraints defined by the model used affects the kinds of behaviors learnt under the prior. A model that can capture the temporal structure present in the training task is \textit{more likely} to generate the target sequence required in the transfer task. We analyze this and the general behaviors captured under the \textit{priors} in greater detail below.
% Therefore a model that fits more closely to that space of trajectories has an advantage during transfer. 

\subsubsection{Analysis}
To understand why the \bps are useful during training and transfer we first need to clarify what \emph{behaviors} they are actually modelling. In order to do this, we use the MLP prior that was learnt on the training task and generate trajectories from it. These trajectories are compared to 'random' trajectories generated from an untrained Gaussian policy in figure  \ref{fig:visualize_traj}. As the figure shows, the \textit{prior} learns to model a behavior of bouncing between the different targets. Since it does not have access to the task-specific information of \textit{which exact target} to visit next, it instead learns to encode the behavior of visiting targets in general. This 'target-centric' behavior is useful to guide the final policy during training and transfer. 

Next we seek to further explore the difference between the behaviors captured under the LSTM model and the MLP. In order to do this, we again generate trajectories using the learnt LSTM and MLP models and compute the transition dynamics when they visit a specific target. In figure \ref{fig:transition_dynamics}, we plot the probability of visiting target 0 against the last 2 visited targets for each model. As opposed to the MLP prior that visits each target more or less uniformly, the LSTM architecture learns to \emph{capture the underlying transition dynamics} of the domain. This in turn results in a significant boost in performance during transfer where the agent is more likely to see the rewarding sequence (by construction on this task).
%and thus learns to capture the additional structure 
% of the domain. In contrast, the MLP prior visits each target more or less uniformly. 

% Therefore the \textbf{choice} of \bp model plays an important role in the space of trajectories that the prior learns to capture. 
It is important to note that restricting the space of trajectories that the prior explores is only advantageous if that space also captures the \textit{solution space} of the task we are ultimately interested in solving. In other words, there is a tradeoff between generality and efficacy of the prior. A prior over trajectories that is 'uniform' in that it assigns equal mass to \emph{all possible trajectories} will be of limited use since it does not capture any of the underlying \textit{task structure}.
%may be too spread out to be of much use.
% \dhruva{Should we mention this here? It would be more easily digested with the negative transfer task perhaps. In general perhaps we should consider a negative transfer result as well?}

\begin{figure}%
    \centering
    \includegraphics[scale=0.26]{figures/set_1/transition_dynamics_set_1.png}
    \caption{\textbf{Transition dynamics} generated under different \bp models to visit target 0. Each point on the x-axis indicates the indices of the last two targets visited. On the y-axis we plot the probability of visiting target 0 for each transition sequence.}
    \label{fig:transition_dynamics}
    % \begin{subfigure}{0.5\textwidth}
    % \centering
\end{figure}

\begin{table}[t]
\scriptsize
% \footnotesize
% \small
\centering
\begin{tabular}{ | m{2.3cm} | m{2.5cm}| m{1.6cm} |  m{1.2cm} |  m{2cm} | m{2cm} |} 
 \hline
 \textbf{Task Name} & \textbf{Description} & \textbf{Body} & \textbf{Action Dim.} & \textbf{Obs.} & \textbf{Obs. to \textit{Prior}} \\
 \hline\hline
 
 \textit{Navigation Easy} & Visit targets in a sequence where the sequence is history dependent. & PointMass / Ant & 2/8 & Proprio + Targets + next target index & Proprio + targets \\ 
 \hline
 
 \textit{Navigation Hard} & Visit targets in order. & PointMass / Ant & 2/8 & Proprio + Targets & Proprio + Targets \\ 
 \hline  
 
 \textit{Locomotion (Humanoid)} & Follow a moving target  & Humanoid & 23 & Proprio +
  Target location & Varies (See text) \\ 
 
 \hline
 
 \textit{Locomotion (Ant)} & Go to one of 3 targets  & Ant & 8 & Proprio + Targets + Index of goal & Varies (See text) \\ 

 \hline
 
 \textit{Locomotion (Gaps)*} & Move forward and jump across a variable length gap. & Ant & 8 & Proprio + Global position + Gap length & Proprio \\ 

 \hline
 
 \textit{Locomotion and Manipulation} & Move a box to a specified target and then move to another target.  & Ant & 8 & Proprio + Box + Targets + Task encoding & Varies (See text) \\ 
 
 \hline
 
 \textit{Manipulation (1 box, 1 target)*} & Move a box to a target location.  & Ant & 8 & Proprio + Box + Targets + Task encoding & Proprio + Box \\
 
 \hline
 
 \textit{Manipulation (1 box, 3 target)*} & Move a box to one of 3 target locations.  & Ant & 8 & Proprio + Box + Targets + Task encoding & Proprio + Box \\ 
 
 \hline
 
 \textit{Manipulation (2 box, 2 target)*} & Move one of two boxes to one of 2 target locations.  & Ball & 2 & Proprio + Boxes + Targets + Task encoding & Proprio + Boxes \\ 
 
 \hline
 
 \textit{Manipulation (2 box gather)*} & Move two boxes close together.  & Ball & 2 & Proprio + Boxes + Targets + Task encoding & Proprio + Boxes \\ 
 \hline
 
\end{tabular}
\caption{\textbf{List of Tasks} A short summary of tasks used along with the information asymmetry used to train the \bp. Tasks marked with a '*' are considered in section \ref{sec:hier_experiments}. A more complete description is presented in Appendix \ref{appendix:tasks}.}
\label{table:task_list}
\end{table}

% Experiments on the flat priors.
\subsection{Effect of Information Asymmetry}

\subsubsection{Locomotion and Manipulation Task}
\label{sec:info_asym_1}
In the previous section, we analyzed how different modeling constraints can affect the kinds of behaviors learnt by the \textit{priors}. In this section, we instead focus on how \emph{information constraints} with the same model affect the behaviors learnt and hence the performance of different \textit{priors} during training. 

We focus our discussion for this part on the \textit{Locomotion and Manipulation} task (which is also considered in the hierarchical setting in section \ref{sec:info_asym_2}) but expand this to include a range of other tasks in section \ref{sec:info_asym_rest}. 

This task involves the agent, a box and two goal locations. In order to solve the task, the agent must move to the box to one of the goals (manipulation) and then move to the other goal (locomotion). The agent receives a reward of +10 for successfully accomplishing either sub-task and an additional bonus  of +50 when it solves both. 
For this task we use an 8-DoF ant walker as shown in Figure \ref{fig:task_bodies}a.

Apart from the proprioceptive information that contains the relative joint positions and velocities of the agent's body (refer to Appendix \ref{appendix:bodies}), the agent also receives the location of the goals, the location of the box and the index of goal it must push the box to. There are therefore many choices of subsets of information that can be sent to the \textit{prior} here and the kinds of behaviors that it can capture will depend on the information it has access to. For instance the \textit{prior} cannot capture the behavior of interacting with the box if it isn't provided the box information. On the other hand, a prior with access to all of the same information as the policy will learn to mimic the policy and lose the regularizing effect created by the information asymmetry. We examine whether this impacts performance on this task.
% In general, a \textit{prior} with a more restricted information set would capture a more general space of behaviors and may be less useful for training the policy. On the other hand, a prior with access to the full set of information would capture the same set of solutions as the policy and be of limited use. This task presents an interesting example to study this trade-off and we consider it again for structured priors in section \ref{sec:hier_experiments}.
% For this task we used additional encoding networks for each input sub-component as we found this sped up learning (more details in Appendix \ref{appendix:experiment_details}).

\begin{figure}%
    \centering
    \includegraphics[width=\linewidth]{figures/set_1/info_asym_mbgtt.png}
    \caption{\textbf{Effect of information asymmetry.} Effect of learning with different levels of information asymmetry on the \textit{Locomotion and Manipulation} task.}
    \label{fig:info_asym_mbgtt}
    % \begin{subfigure}{0.5\textwidth}
    % \centering
\end{figure}

% We experiment with various settings of information asymmetry between the \bp and the agent policy in figure
We present our results in figure \ref{fig:info_asym_mbgtt}. We find a marked difference in performance based on the information that the \bp has access to. We observe that most policies on this task (including training from scratch) can easily get stuck in a local optima where the agent learns to solve the easier locomotion component of the task but never learns about the additional reward for moving the box. However, certain \bps can help regularize against this sub-optimal solution by encouraging useful patterns of behavior. For instance, a prior that has access to \textit{only} proprioceptive information would ostensibly encode the space of trajectories containing primitive gaits or movements.
%relating to the agent moving around in the environment. 
By encouraging the policy to continue to explore in this space, the agent is more likely to continue learning and to see the full task reward. In this case we find that the \bp that has access to both proprioception as well as the location of the box learns the fastest. We hypothesize that this prior could model the space of trajectories related to moving a box around which would be useful to get out of the local optima described above. We revisit this idea in section \ref{sec:hier_experiments} and show an example of a hierarchical prior models this behavior in a similar setting.

\subsubsection{Other Tasks}
\label{sec:info_asym_rest}

\begin{figure}%
    \centering
    \includegraphics[width=\linewidth]{figures/set_1/info_asym_rest.png}
    \caption{\textbf{Effect of information asymmetry.} Effect of learning with different levels of information asymmetry on \textit{Manipulation (1 box, 3 targets)}, \textit{Locomotion (Humanoid)} and \textit{Locomotion (Ant)}.}
    \label{fig:info_asym_rest}
    % \begin{subfigure}{0.5\textwidth}
    % \centering
\end{figure}

In this section, we expand our analysis of the effect of information asymmetry for learning on three more tasks: \textit{Manipulation (1 box, 3 targets)}, \textit{Locomotion (Humanoid)} and \textit{Locomotion (Ant)} (refer to table \ref{table:task_list} for a short summary).
% \begin{itemize}
%     \item \textbf{Manipulate many (Ant)}: The ant must move a box to one of 3 target locations.
%     \item \textbf{Locomotion (Humanoid)}: This is a goal following task with the Humanoid body. The agent is given a goal location that it must reach, at which point a new goal is generated. This continue until the episode times out.
%     \item \textbf{Locomotion (Ant)}: The ant must move to one of 3 target locations.
% \end{itemize}

% The tasks were chosen to cover a range of complexities related to the task and agent body. 
We show our findings in Figure \ref{fig:info_asym_rest}.
We observe that regularizing against a \bp \textbf{always provides a benefit} and \textit{priors} with partial information always perform better than ones with full information. Additionally, \bps with access to only proprioceptive information tend to perform the best in tasks involving just locomotion. Note that this is also true for the complex \textit{Locomotion (Humanoid})} task where a 21-dof humanoid walker must learn to visit a moving target. Our intuition is that providing just proprioceptive information allows for priors that model trajectories containing primitive movement patterns.
% This is consistent with the intuition described earlier that this allows for priors that model general trajectory spaces that contain primitive movement patterns. 

We analyze this in greater detail in figure \ref{fig:gtt_humanoid_kl} for the \textit{Locomotion (Humanoid)} task by studying the KL divergence between the \textit{prior} and policy as the agent visits different goals as shown in in figure \ref{fig:gtt_humanoid_targets}.
% In figure \ref{fig:gtt_humanoid_targets}, we show the trajectory followed by the humanoid in the \textit{Locomotion (Humanoid)} task where the target moves when the agent reaches it. In figure \ref{fig:gtt_humanoid_kl} we plot the KL divergence between the policy and the \bp where the \bp here only gets proprioceptive information. 
As the figure illustrates, the \bp and the policy match quite closely (and so the KL is low) until the agent reaches a target. At this point, the policy changes to a new pattern of movement in order to change direction and go toward the new target location. We observe spikes in the KL divergence \emph{precisely when new targets} are chosen. As the humanoid settles into a new movement pattern, we observe the KL once again reduces and this sequence repeats for each of the targets. Furthermore, in figure \ref{fig:gtt_humanoid_prior}, we generate trajectories under the learnt \textit{prior} from the same initial position and observe that the \bp captures forward movement in different directions with occasional sharp turns. These results indicate that movement, even for a complex 21-dof humanoid robot, involves a locomotive pattern that mostly depends on the \emph{current configuration of the body}. This also demonstrates the ability of our method to learn quite complex and powerful primitive behaviors. 

% This result indicates that moving between targets involves a locomotive pattern that mostly depends on the configuration of the body and this pattern is precisely the \textit{behavior} that the prior learns to capture. 
% the movements required to transition between targets are consistent and only depend on the configuration of the body. This is precisely the behavior that the \textit{prior} learns to model.
% These eventually reduce as the \bp adapts to the new movement pattern (after completing a turn say), indicating that the prior does indeed encode movements.
% Used to be width=-.45\linewidth
\begin{figure}%
    \centering
    \subfloat[Trajectory of humanoid visiting targets in the \textit{Locomotion (Humanoid)} task. \label{fig:gtt_humanoid_targets}]{{\includegraphics[scale=0.14]{figures/set_1/gtt_humanoid_targets.png} }}%
    \qquad
    \subfloat[Deviation of policy from the \bp in terms of KL divergence. \label{fig:gtt_humanoid_kl}]{{\includegraphics[scale=0.14]{figures/set_1/gtt_humanoid_kl.png} }}%
    \qquad
    \subfloat[Trajectories generated by the \bp. \label{fig:gtt_humanoid_prior}]{{\includegraphics[scale=0.14]{figures/set_1/gtt_humanoid_prior.png} }}%    
    \caption{\textbf{Analysis of the \textit{Locomotion (Humanoid)} task}. The spikes in KL divergence in the center align with the change in target as on the left; this is consistent with the idea that the \bp encodes primitive movement patterns. Trajectories generated under the \bp result in forward movement with occasional turns as shown on the right figure.}
    \label{fig:gtt_humanoid}
\end{figure}

==> older_version/hierarchical_experiments.tex <==
\section{Experiments with structured priors}
\label{sec:hier_experiments}

In this section, we analyze structured \bps on a range of control domains. To begin with, we extend the analysis of sections \ref{sec:toy_domain_1} and \ref{sec:info_asym_1} to incorporate structured priors. Finally, we compare the performance of structured and unstructured models for training and transfer. Unless otherwise specified, all the structured priors we consider for this part include a shared lower level policy as described in section \ref{sec:structured_models}.

\subsection{Toy Domain: Pointmass on Grid}
We now extend the analysis for section \ref{sec:toy_domain_1} where a pointmass must visit a sequence of targets on a grid to include hierarchical models. In the hierarchical formulations, the input observation is passed into the higher level whose outputs are the mean and variance of a Gaussian distribution. A higher level latent $z$ is sampled from this distribution and passed into the lower level controller. Both the higher and lower levels also receive the location of the agent and targets as input. We experiment with two types of \bps: \textit{Hier. MLP} and \textit{Hier. LSTM} where the higher level is an MLP or an LSTM respectively. This approach is contrasted with unstructed priors in figure \ref{fig:structured_priors_descr}.

\begin{figure}%
    \centering
    \subfloat[Learning with structured priors on Hard Task\label{fig:easy_set_2}]{{\includegraphics[width=0.45\linewidth]{figures/set_2/easy_task_set_2.png} }}%
    \qquad
    \subfloat[Transfer of structured priors to hard task\label{fig:hard_set_2}]{{\includegraphics[width=0.45\linewidth]{figures/set_2/hard_task_set_2.png} }}%
    \caption{\textbf{Learning and transfer} with structured \bps on the toy domain.}
    \label{fig:pointmass_results_2}
\end{figure}


We compare the performance of structured and unstructured priors during training and transfer in Figure \ref{fig:pointmass_results_2}. All \bps boost learning performance on this task and we observe no significant difference during training of each of the priors. In figure \ref{fig:hard_set_2}, we compare the performance of the structured and unstructured models during transfer to the hard task. Here we find the hierarchical LSTM model learns to solve the task almost immediately. Since the lower level prior (and hence policy) is fixed during transfer, there are fewer parameters to train for the hierarchical models which could explain the speed in learning. As described in section \ref{sec:toy_domain_1}, priors that can capture the latent dynamics of the task perform better during transfer. We illustrate this using table  \ref{table:reward_rollout_kl_pointmass}, where we record the average returns generated by rolling out the trained priors on the transfer task for a 100 episodes. As we hypothesized, priors with memory (LSTM and hier. LSTM) are more likely to visit the rewarding sequence and generate much higher returns during exploration. Rollouts under these priors also have a lower KL divergence against the true underlying dynamics of the task as illustrated by figure \ref{fig:transition_dynamics_2} as well.

Finally, we compare the performance of all models on a variant of this task that uses the 8-dof 'ant' walker in figure \ref{fig:ant_toy_results}. Our results are consistent on this harder task, where we observe models with memory significantly outperform others during transfer. In the structured case, we expect the primitive movement like behaviors are encoded in the lower level policy.

% and measure the empirical KL of the dynamics against the true transition dynamics of the easy task. 

% and observe the LSTM priors outperform the MLP ones by some margin. We also record the KL between the true transition dynamics of the task and the empirical dynamics (as in figure \ref{fig:transition_dynamics_2}) and observe that it is lowest for priors which have the LSTM.

\begin{figure}%
    \centering
    \includegraphics[width=0.9\linewidth]{figures/set_2/transition_dynamics_set_2.png}
    \caption{\textbf{Transition dynamics for first target} generated under structured \bp models. Each point on the x-axis indicates the indices of the last two targets visited. On the y-axis we plot the probability of visiting the target for each transition sequence.}
    \label{fig:transition_dynamics_2}
\end{figure}

\begin{figure}%
    \centering
    \subfloat[Learning with structured priors on easy task (Ant) \label{fig:ant_easy_set_2}]{{\includegraphics[width=0.45\linewidth]{figures/set_2/easy_task_ant_set_2.png} }}%
    \qquad
    \subfloat[Transfer of structured priors to hard task (Ant) \label{fig:ant_hard_set_2}]{{\includegraphics[width=0.45\linewidth]{figures/set_2/hard_task_ant_set_2.png} }}%
    \caption{\textbf{Learning and transfer} on toy domain with the 'Ant' walker.}
    \label{fig:ant_toy_results}
\end{figure}

\begin{table}
\centering
\begin{tabular}{ | m{4cm} | m{2cm}| m{2cm} |  m{2cm} |  m{2cm} |} 
 \hline
 \textbf{Model} & \textbf{Hier. LSTM} & \textbf{Hier. MLP} & \textbf{LSTM} & \textbf{MLP} \\
 \hline
  \hline
 
 \textbf{Return} & \textbf{81.28} & 43.82 & \textbf{82.00} & 33.94 \\ 
 \hline
 \textbf{KL} & \textbf{0.262} & 0.760 & \textbf{0.191} & 0.762 \\ 
 
 \hline

\end{tabular}
\caption{\textbf{Average return and KL}. For each pre-trained model, we compute statistics by rolling out the \textit{prior} on the hard task (Averaged across a 100 episodes for 5 seeds).}
\label{table:reward_rollout_kl_pointmass}
\end{table}

In the remainder of this section, we explore this idea further and show how such primitives when encoded in the lower level \bp can be used for training and transfer. Since our focus is on the behaviors encoded in the lower level, in what follows, we consider parameter-free higher level (HL) policies. Specifically we consider higher levels that are either:
%
\textbf{Independent isotropic Gaussian.} $\pi^H_0(z_t | x_t) = \mathcal{N}(z_t | 0, 1)$, where the HL \bp assumes the abstract actions to be context independent or 
%
\textbf{AR(1) process.} $\pi^H_0(z_t | x_t) = \mathcal{N}(z_t | \alpha z_{t-1}, \sqrt{1-\alpha^2} )$, where the HL \bp is a first-order auto-regressive process with a fixed parameter $0 \leq \alpha < 1$ chosen to  ensure a marginal distribution $\mathcal{N}(0,1)$. This allows for more structured temporal dependence among the abstract actions.

We find these models are more stable for learning and are sufficient for the kinds of tasks we consider in the remainder of the text. 

\subsection{Effect of Information Asymmetry}

\subsubsection{Locomotion and Manipulation Task}
\label{sec:info_asym_2}
Similar to section \ref{sec:info_asym_1}, in this section we showcase how partial information can be advantageous for a \bp. We once again consider the \textit{Locomotion and Manipulation} task (see Table \ref{table:task_list}) with the Ant. However for this experiment, we consider structured models with a shared lower level policy and an isotropic gaussian higher level prior. As in section \ref{sec:info_asym_1} we study the effect of various kinds of information asymmetry between the higher and lower level. In this case, to solve the task, information withheld from the lower level would need to be \textit{encoded} in the higher level latent $z$.

\begin{figure}%
    \centering
    \includegraphics[width=\linewidth]{figures/set_2/info_asymm_mbgtt_hier.png}
    \caption{\textbf{Effect of information asymmetry} with structured models on the 'Locomotion and Manipulation' task.}
    \label{fig:info_asym_mbgtt_hier}
    % \begin{subfigure}{0.5\textwidth}
    % \centering
\end{figure}

As figure \ref{fig:info_asym_mbgtt_hier} illustrates, we see a similar effect of information asymmetry as in section \ref{sec:info_asym_1}. Specifically, \bps with partial information perform better than ones with full information. Additionally, providing proprioceptive as well as box information works best followed by a prior with only proprioceptive information. 

To better understand this, we sample random latent $z$s from our higher level prior and feed them into the lower level policies to generate the trajectories in figure \ref{fig:ant_rollout}. We observe that the \textit{priors} with access to the box information show a more \textit{goal-directed} behavior with  the ant pushing the box around more frequently which is likely a good exploration strategy for this task.

% Therefore, while hiding information seems to be universally important for good performance of the \bp, often hiding the \textit{right kind} of information can lead to \bps which are better at exploiting the structure in the task.

\begin{figure}%
    \centering
    \includegraphics[width=\linewidth]{figures/set_2/ant_exploration_trajectories.png}
    \caption{\textbf{Effect of information asymmetry on exploration} A visualization of the motion of the ant (red) and the box (blue) under random latent samples fed to a lower level policy with a) just proprioceptive information and b) proprioceptive and box information.}
    \label{fig:ant_rollout}
\end{figure}

\subsection{Comparison of structured and unstructured priors}
We now assess the performance of structured and unstructured \bp models during training and transfer on a range of control tasks. To begin with, we consider the effect of various \bps during training three tasks: \textit{Locomotion (Ant)}, \textit{Manipulation (1b, 1t)} and \textit{Manipulation (2b, 2t)} (refer to table \ref{table:task_list} for a short summary and the information asymmetry used). 

We illustrate our results in figure \ref{fig:speedup_hier}. We observe that \bps \textbf{always} result in a speedup in learning. Furthermore, we find that hierarchical \bp models tend to outperform the unstructured ones and this gap increases for the more complex tasks (\textit{Manipulation (2b, 2t)}). We also found no significant difference between using an isotropic Gaussian prior or an AR-1 prior at the higher level.

\begin{figure}%
    \centering
    \includegraphics[width=\linewidth]{figures/set_2/speedup_hierarchy.png}
    \caption{\textbf{Learning performance} with different \bps on the \textit{Locomotion (Ant)}, \textit{Manipulation (1b, 1t)} and \textit{Manipulation (2b, 2t)} tasks.}
    \label{fig:speedup_hier}
    % \begin{subfigure}{0.5\textwidth}
    % \centering
\end{figure}

%An important point to note is that the behaviors captured by our \bps are more \textit{general} as a result of information asymmetry. We exploit this 
In a second set of experiments, we consider a \textit{transfer} scenario where we regularize against pre-trained \textit{priors} on a new task.
We consider two transfer tasks: \textit{Manipulation (1b, 3t)} where we transfer from a task with fewer targets ((\textit{Manipulation (1b, 1t)}) and \textit{Manipulation (2b, gather)} where we transfer from a task with a different objective (\textit{Manipulation (2b, 2t)}). In figure \ref{fig:transfer_hier} where we compare the performance of a pre-trained prior against learning the task from scratch with an \textit{untrained prior}(Note that our previous results indicate this is faster than learning with \textit{no prior} at all.).
In general, we observe a significant boost in performance when regularizing against \bps. Additionally, the structured models perform significantly better during transfer. This highlights an important advantage of structure - the information captured by the lower level prior is directly shared with the transfer policy.
However on the \textit{Manipulation (2b, gather)} we observe the MLP prior performs worse during transfer than learning from scratch. Further analysis showed that this was the result of two pretraining seeds that never took off during transfer.

\begin{figure}%
    \centering
    \includegraphics[width=\linewidth]{figures/set_2/transfer_hier.png}
    \caption{\textbf{Transfer performance} with various \bps on \textit{Manipulation (1b, 3t)} and \textit{Manipulation (2b, gather).}}
    \label{fig:transfer_hier}
    % \begin{subfigure}{0.5\textwidth}
    % \centering
\end{figure}

\subsection{Separate low level modules}
Finally in this section we consider an example scenario where a separate lower level prior $\pp^L$ may be advantageous to learn new skills.
%All of the experiments considered thus far share the lower level policy between the \bp and the policy.
%%We consider an example task as shown in figure \ref{fig:transfer_hier_split} where the transfer domain requires \textit{new skills}. 
In our example, we train a controller on the \textit{Locomotion (Ant)} task but transfer it to the \textit{Locomotion (Gaps)} task. The transfer domain consists of a room with a gap of variable length in the center of it. The agent is rewarded for moving forward at each time step but must learn to jump across larger gaps to consistently solve the task. In this example, the \textit{prior} with a shared lower level does not capture the behaviors required to solve the task optimally. As shown in figure \ref{fig:transfer_hier_split}, we can adapt the skills of the \bp into a new lower level policy using the model described in section \ref{sec:hier_experiments}.

\begin{figure}%
    \centering
    \includegraphics[width=.7\linewidth]{figures/set_2/transfer_split.png}
    \caption{\textbf{Skill adaptation for hierarchical models} using separate lower level controllers on the \textit{Locomotion (Gap)} task.}
    \label{fig:transfer_hier_split}
    % \begin{subfigure}{0.5\textwidth}
    % \centering
\end{figure}

==> older_version/hierarchical_experiments_v2.tex <==
\section{Experiments with structured priors}
\label{sec:hier_experiments}
% Currently too dry - needs more intuition.
% For each env. - why do we want to study it? (Can say described before).
%  and then what is the interesting property that comes out from the expt.
% AR-1 connect to NPMP for why we study it. 
%
%  KL Divergence for with DISTRAL and Gaussian prior - 11.35 and 2.64. (5 seeds; 100 eps)
% 
In this section, we analyze the performance of structured \bps on a range of control domains. Our goal is to understand whether \emph{hierarchical priors} are more efficient at capturing the underlying structure in our tasks and to study the potential benefits of partial parameter sharing between $\qp$ and $\pp$. We begin by extending the analysis on the 'Sequential Navigation' task in section \ref{sec:toy_domain_1} to study how well modular policies can capture behaviors on a task with multiple levels of structure. Next, we carry out an ablation analysis similar to the one in section \ref{sec:info_asym_1} to study how information asymmetry in modular policies affects learning. Finally, we compare structured and unstructured models of behavior across a range of 'Locomotion' and 'Manipulation' tasks to demonstrate how they can be used to speedup training and transfer.
% Finally, we compare the performance of structured and unstructured models for training and transfer on a range of 'Locomotion' and 'Manipulation' tasks  
Unless otherwise specified, all the structured priors we consider for this part include a shared lower level policy as described in section \ref{sec:structured_models}. In the hierarchical formulation, the higher level outputs the mean and variance of a Gaussian distribution from which the latent $z$ is sampled to be passed into the lower level controller.

\subsection{Sequential Navigation}
In section \ref{sec:toy_domain_1}, we demonstrated how the choice of model for the \textit{prior} can affect the behaviors captured on a Sequential Navigation task. This task involves structure at various levels - goal-directed locomotion behavior and long-horizon behavior due to some sequences being more likely to be generated. In this section we extend this analysis to structured priors where we are also interested in what kinds of behaviors are captured in the different levels of the hierarchy and how this in turn affects learning. Additionally, we consider a more complex form of this task with the 'Ant' walker.
With a similar intuition as in section \ref{sec:toy_domain_1}, we consider two types of models for the higher level for this task, based on their ability to capture correlations across time: \textit{Hier. MLP} and \textit{Hier. LSTM}. For all our experiments we used an LSTM critic and an LSTM for both posterior higher level policies and MLPs for the lower level policies (full details can be found in appendix \ref{appendix:experiment_details}. We use a similar information asymmetry to section \ref{sec:toy_domain_1} but here both the higher level prior and shared lower level do not have access to task-specific information.

\begin{figure}%
    \centering
    \subfloat[Learning with structured priors on the easy Task\label{fig:easy_set_2}]{{\includegraphics[scale=0.25]{figures/set_2/easy_task_set_2.png} }}%
    \qquad
    \subfloat[Transfer of structured priors to hard task\label{fig:hard_set_2}]{{\includegraphics[scale=0.25]{figures/set_2/hard_task_set_2.png} }}%
    \caption{\textbf{Learning and transfer} with structured \bps on the 'Sequential Navigation' task.}
    \label{fig:pointmass_results_2}
\end{figure}

As figure \ref{fig:pointmass_results_2} shows \emph{both} structured and unstructured \bps improve learning speed on this task. Thus the intuition that \bps can help guide learning continues to hold in the structured case. Interestingly there seems to be a slight advantage of using the \textit{Hier. MLP} prior in this case. While it isn't entirely clear why this may be it is clear that there may be a benefit of using structured models during training and that it may be easier to learn hierarchical MLP priors than hierarchical LSTMs.
% This hints at the possibility that this structure is easier to learn than the \textit{Hier. LSTM} while still providing the modeling benefits of using latent variable models.
In figure \ref{fig:hard_set_2}, we compare the performance of the structured and unstructured models during transfer to the hard task. Our results are consistent with that in section \ref{fig:hard_set_1} in the sense that the priors that can model the temporal structure in the task (LSTM and Hier. LSTM) are more \emph{likely} to generate the rewarding sequence during transfer and hence learn significantly faster. We illustrate this using table  \ref{table:reward_rollout_kl_pointmass}, where we record the average returns generated on the transfer task over a 100 episodes using the trained priors. As we hypothesized, priors with memory (LSTM and hier. LSTM) are more likely to visit the rewarding sequence and thus generate much higher returns during early exploration. Trajectories generated under these priors also have a lower KL divergence against the true underlying dynamics of the task which is illustrated qualitatively in figure \ref{fig:transition_dynamics_2} and quantitatively in table  \ref{table:reward_rollout_kl_pointmass}.
Finally, since the lower level prior (and hence policy) is fixed during transfer, there are fewer parameters to train for the hierarchical models which could explain why the structured models perform better at transfer.

A possible advantage of structured models is in their ability to model different \emph{aspects} of the behavior in each layer of the hierarchy. With this in mind, we consider a version of this task with the same task dynamics but using the more complex 'ant' body. This version of the task which we call \emph{Sequential Navigation (Ant)} allows us to test whether a split between 'task' behaviors in the higher level and 'movement' behaviors in the lower level could prove advantageous. We show our results in figure \ref{fig:ant_toy_results}. During training, there does seem to be an advantage of using the \textit{Hier. MLP prior} as opposed to the \textit{MLP} prior. Since neither of these models can capture the underlying dynamics of the task, this indicates that the advantage here comes from the ability of the structured model to better capture the complexity of the body. Interestingly this difference is not as prominent when compared to the \textit{LSTM} prior - indicating that the memory dependent architecture may have a similar advantage.

\dhruva{Rethink this last bit. The explanations are inconsistent and a bit over the place - What exactly do we want to say about these tasks?}
% Our results are consistent on this harder task, where we observe models with memory significantly outperform others during transfer. In the structured case, we expect the primitive movement like behaviors are encoded in the lower level policy.

% and measure the empirical KL of the dynamics against the true transition dynamics of the easy task. 

% and observe the LSTM priors outperform the MLP ones by some margin. We also record the KL between the true transition dynamics of the task and the empirical dynamics (as in figure \ref{fig:transition_dynamics_2}) and observe that it is lowest for priors which have the LSTM.

\begin{figure}%
    \centering
    \includegraphics[scale=0.26]{figures/set_2/transition_dynamics_set_2.png}
    \caption{\textbf{Transition dynamics for first target} generated under structured \bp models. Each point on the x-axis indicates the indices of the last two targets visited. On the y-axis we plot the probability of visiting the target for each transition sequence.}
    \label{fig:transition_dynamics_2}
\end{figure}

\begin{figure}%
    \centering
    \subfloat[Learning with structured priors on easy task (Ant) \label{fig:ant_easy_set_2}]{{\includegraphics[scale=0.25]{figures/set_2/easy_task_ant_set_2.png} }}%
    \qquad
    \subfloat[Transfer of structured priors to hard task (Ant) \label{fig:ant_hard_set_2}]{{\includegraphics[scale=0.25]{figures/set_2/hard_task_ant_set_2.png} }}%
    \caption{\textbf{Learning and transfer} on \textit{Sequential Navigation (Ant)}}
    \label{fig:ant_toy_results}
\end{figure}

\begin{table}
\centering
\begin{tabular}{ | m{4cm} | m{2cm}| m{2cm} |  m{2cm} |  m{2cm} |} 
 \hline
 \textbf{Model} & \textbf{Hier. LSTM} & \textbf{Hier. MLP} & \textbf{LSTM} & \textbf{MLP} \\
 \hline
  \hline
 
 \textbf{Return} & \textbf{81.28} & 43.82 & \textbf{82.00} & 33.94 \\ 
 \hline
 \textbf{KL} & \textbf{0.262} & 0.760 & \textbf{0.191} & 0.762 \\ 
 
 \hline

\end{tabular}
\caption{\textbf{Average return and KL}. For each pre-trained model, we compute statistics by generating trajectories under the \textit{prior} on the hard task (Averaged across a 100 episodes for 5 seeds).}
\label{table:reward_rollout_kl_pointmass}
\end{table}

% In the remainder of this section, we explore this idea further and show how such primitives when encoded in the lower level \bp can be used for training and transfer. Since our focus is on the behaviors encoded in the lower level, in what follows, we consider parameter-free higher level (HL) policies. Specifically we consider higher levels that are either:
So far we have demonstrated that our method for training structured models of behavior are at least on par with unstructured \bps and can improve learning speed on tasks with a temporally correlated structure. In the remainder of this section we will shift our focus to the 'Locomotion' and 'Manipulation' tasks introduced in section \ref{sec:experiments}. Our goal is to study if there are potential benefits to the hierarchical decomposition in terms of partial parameter sharing of the lower level or the ability of these models to capture richer distributions. 
% the structure in these arises from the repetitive patterns of interaction between the agent and environment. 

% In the hierarchical setting, we are interested in capturing these behaviors in the lower level policy since this is \emph{shared} between $\qp$ and $\pp$ and could have additional benefits during transfer.
% We therefore consider simpler models for the higher level prior $\pp_H$ including:
In what follows we consider two models for the higher level prior $\pp^H$:
%
\textbf{Independent isotropic Gaussian.} $\pi^H_0(z_t | x_t) = \mathcal{N}(z_t | 0, 1)$, where the HL \bp assumes the abstract actions to be context independent or 
%
\textbf{AR(1) process.} $\pi^H_0(z_t | x_t) = \mathcal{N}(z_t | \alpha z_{t-1}, \sqrt{1-\alpha^2} )$, where the HL \bp is a first-order auto-regressive process with a fixed parameter $0 \leq \alpha < 1$ chosen to  ensure the variance of the noise is marginally distributed according to $\mathcal{N}(0, I)$. We include this model since it showed promising results in \cite{merel2018neural} and could allow for temporal dependence among the abstract actions. However in our results we found no significant advantage of using this over the isotropic Gaussian.

We find these models are more stable to train than the \textit{Hier. MLP and LSTM} priors considered previously and are sufficient for the kinds of tasks we consider in the remainder of the text. Finally the only unstructured model we consider going forward is the MLP prior since the tasks do not require memory.

\subsection{Effect of Information Asymmetry}

\subsubsection{Locomotion and Manipulation Task}
\label{sec:info_asym_2}
As described in section \ref{sec:hierarchy:info_asym}, we expect information asymmetry between the different levels of the hierarchy to play an important role in shaping the learning dynamics; an idea which we demonstrate empirically in this section.
For our analysis, we once again consider the \textit{Locomotion and Manipulation} task (see Table \ref{table:task_list}) as in section \ref{sec:info_asym_1}. For this experiment, we consider structured models with a shared lower level policy and an isotropic gaussian higher level prior. 
% As in section \ref{sec:info_asym_1} we study the effect of various kinds of information asymmetry between the higher and lower level. In this case, to solve the task, information withheld from the lower level would need to be \textit{encoded} in the higher level latent $z$.
\begin{figure}%
    \centering
    \includegraphics[width=\linewidth]{figures/set_2/info_asymm_mbgtt_hier.png}
    \caption{\textbf{Effect of information asymmetry} with structured models on the 'Locomotion and Manipulation' task.}
    \label{fig:info_asym_mbgtt_hier}
    % \begin{subfigure}{0.5\textwidth}
    % \centering
\end{figure}

As figure \ref{fig:info_asym_mbgtt_hier} illustrates, we see a similar effect of information asymmetry as in section \ref{sec:info_asym_1}. Specifically, \bps with partial information perform \emph{better} than ones with access to full information and in fact we see a pattern very similar to the one from section \ref{sec:info_asym_1}. As described previously, this task includes a local optima where agents that learn to solve the easier 'Locomotion' component of the task do not go on to learn both components and hence solve the full task. The lower level policies with partial information (only proprioception or proprioception and box) model a general space of trajectories similar to the \textit{prior} in section \ref{sec:info_asym_1}. However as opposed to the previous case where the prior served as a useful regularizer, here the regularizing effect comes into play due to the \emph{noise in sampling $z$s} that is generated by the higher level prior $\pp^H$. As opposed to 'primitive action' noise that is considered in \citet{haarnoja2018soft}, noise in the the higher level $z$ corresponds to an actual behavior in the lower level and thus translates into a more structured form of exploration.
\dhruva{does the last paragraph make sense? Maybe needs more handholding?}

In order to understand this idea of structured exploration better, we conduct an experiment using trained priors from figure \ref{fig:info_asym_mbgtt_hier} where the lower level has access to - a) only proprioception and b) proprioception and box information. Using these, we sample random latent $z$s from our higher level prior and feed them into the lower level to generate the trajectories as shown in figure \ref{fig:ant_rollout}. The \textit{prior} with only proprioceptive information learns to model movement behaviors in the lower level and thus random exploration in the higher level latent space leads to more structured trajectories of movement in different directions. In contrast, we observe that the \textit{prior} with access to both proprioception and box information shows a more \textit{goal-directed} behavior where the agent moves toward the box and pushes it. This latter behavior is likely to be useful to get out of the local optima in the 'Locomotion and Manipulation' task where agents do not learn to push the box to the target.
% Therefore, while hiding information seems to be universally important for good performance of the \bp, often hiding the \textit{right kind} of information can lead to \bps which are better at exploiting the structure in the task.
\begin{figure}%
    \centering
    \includegraphics[scale=0.25]{figures/set_2/ant_exploration_trajectories.png}
    \caption{\textbf{Effect of information asymmetry on exploration} A visualization of the motion of the ant (red) and the box (blue) under random latent samples fed to a lower level policy with a) just proprioceptive information and b) proprioceptive and box information.}
    \label{fig:ant_rollout}
\end{figure}

\subsection{Comparison of structured and unstructured priors}
In the discussion so far we have demonstrated a method to train structured and unstructured \textit{priors} and studied some of their properties in some detail. In this section we bring all of this together and compare how structured and unstructured \textit{priors} fare during training and transfer on a range of 'Locomotion' and 'Manipulation' tasks. To begin with, we consider the effect of during training on three tasks: \textit{Locomotion (Ant)}, \textit{Manipulation (1 box, 1 target)} and \textit{Manipulation (2 boxes, 2 targets)} (refer to table \ref{table:task_list} for a short summary and the information asymmetry used). 

We illustrate our results in figure \ref{fig:speedup_hier}. We observe that \bps \textbf{always} result in a speedup in learning. Furthermore, we find that hierarchical \bp models tend to perform as well or better than the unstructured ones and this gap increases for the more complex tasks (\textit{Manipulation (2b, 2t)}). In contrast to the findings of \citet{merel2018neural}, we found no significant difference between using an isotropic Gaussian prior or an AR-1 prior at the higher level. This is not too surprising since the tasks we consider here do not require memory to be solved.

\begin{figure}%
    \centering
    \includegraphics[width=\linewidth]{figures/set_2/speedup_hierarchy.png}
    \caption{\textbf{Learning performance} with different \bps on the \textit{Locomotion (Ant)}, \textit{Manipulation (1b, 1t)} and \textit{Manipulation (2b, 2t)} tasks.}
    \label{fig:speedup_hier}
    % \begin{subfigure}{0.5\textwidth}
    % \centering
\end{figure}

A key aspect behind the introduction of the structured models was in their ability to better capture complex distributions. In order to study whether this effect holds true empirically, we computed the average KL divergence between the posterior and \textit{prior} policy on the \textit{Manipulation (1 box, 1 target)} across 5 seeds and a 100 episodes. Values of 11.35 and 2.64 for the Hier. MLP and MLP prior are consistent with the idea that the latent variable formulation  provides a better \textit{prior} over the trajectory distribution and thus allows for a more favorable trade-off between KL and task reward. 

Figure \ref{fig:distrbn_comparison} helps to demonstrate this point qualitatively. In the figure, for a \emph{fixed $x_D$} (where $x_D$ is the 'goal agnostic' information subset passed into the lower level), we sample different values of $x_G$ (the 'goal specific' information) from the initial state distribution and generate samples under the posterior policy. In effect, this represents the empirical action distribution for the policy marginalized over different goals. We show this distribution for a particular action dimension with the unstructured MLP model in figure \ref{fig:distrbn_distral}. Clearly there are multiple optimal modes of optimal behavior based on the 'goal context' which a simple uni-modal Gaussian cannot accurately capture. In fact, it spreads the probability mass across the different modes which may in some cases even be detrimental. In contrast, the hierarchical prior of figure \ref{fig:distrbn_hierarchical} does a better job of capturing such a distribution since the action distribution $\pp^L$ is conditioned on samples from the higher level prior $\pp^H$ in this case.

\begin{figure}%
    \centering
    \subfloat[ \label{fig:distrbn_distral}]{{\includegraphics[scale=0.13]{figures/set_2/distribution_distral.png} }}%
    \qquad
    \subfloat[ \label{fig:distrbn_hierarchical}]{{\includegraphics[scale=0.13]{figures/set_2/distribution_hierarchical.png} }}%
    \caption{\textbf{Empirical distributions} for different goals under the posterior and prior distributions for the MLP and Hier. Gaussian models on the \textit{Manipulation (1 box, 1 target} task.}
    \label{fig:distrbn_comparison}
\end{figure}

%An important point to note is that the behaviors captured by our \bps are more \textit{general} as a result of information asymmetry. We exploit this 
Next, we study the effectiveness of \textit{priors} for \textit{transfer}, where we train a policy for the transfer task while regularizing against a fixed pre-trained \textit{prior}. Since the \textit{priors} capture a more general set of behaviors and require only a subset of the task information, the same \textit{prior} can be useful on new tasks which require similar behaviors.
With this in mind, we consider two transfer tasks: \textit{Manipulation (1box, 3targets)} where we transfer from a task with fewer targets ((\textit{Manipulation (1box, 1targets)}) and \textit{Manipulation (2box gather)} where we transfer from a task with a different objective (\textit{Manipulation (2box, 2targets)}). 

We show our results in figure \ref{fig:transfer_hier} where we compare the performance of regularizing against a pre-trained prior against learning the task from scratch with an \textit{untrained prior} (Note that our previous results indicate this is already faster than learning with \textit{no prior} at all.). For the transfer experiments, we average over 10 seeds for each of the priors (2 seeds for each of the 5 pre-training seeds).
In general, we observe a significant boost in learning speed when regularizing against structured \bps across all transfer tasks. For the hierarchical case, since we share the lower level policies, the behaviors captured under by these during training are \emph{directly transferred} unlike in the case of the \textit{MLP prior} where they must be learnt through the KL reward. This highlights an important advantage of structure - the information captured by the lower level prior is directly shared with the transfer policy.

For the non-structured \textit{MLP prior} we observe it performs \emph{worse} during transfer than learning from scratch on the \textit{Manipulation (2b, gather)} task. On further analysis, we came to realize that this was because some of the seeds from pre-training had not yet converged (see figure \ref{fig:speedup_hier}) and thus the pre-trained priors had not yet captured the \textit{behaviors} needed for transfer. We also plot the performance during transfer when only using the pre-training seeds that had converged (dotted purple line in the figure which is averaged across 6 seeds - 2 seeds each for 3 pretraining seeds). In this case we once again observe that training with the \textit{prior} leads to faster convergence.

\begin{figure}%
    \centering
    \includegraphics[scale=0.25]{figures/set_2/transfer_hier_alternate.png}
    \caption{\textbf{Transfer performance} with various \bps on \textit{Manipulation (1b, 3t)} and \textit{Manipulation (2b, gather).}}
    \label{fig:transfer_hier}
\end{figure}

\subsection{Separate low level modules}
All of the structured models we have considered so far used a lower level policy that was shared between the \textit{prior} $\pp$ and policy $\qp$. In the previous section, we showed how this might be advantageous for transfer since it allows us to directly \textit{reuse} the space of behaviors contained by the lower level prior. In contrast, in the unstructured case, these behaviors would need to be \textit{learnt} through the regularizing effect of the KL reward between the \textit{prior} and the policy. While this is useful in many cases, this also \emph{constrains} the behaviors of the final policy since the lower level prior (and hence policy) is fixed during transfer. In this section, we expand on this point and consider an example where this approach can be limiting. In order to do this, we consider a transfer task \textit{Locomotion (Gaps)} where the agent must learn to \emph{jump} over a variable sized gap that is always at the same location in a straight corridor. The agent is rewarded at each time step for its forward velocity along the corridor. The lower level prior trained from the \textit{Locomotion (Ant)} task contains behaviors for moving forward which is useful to jump over small gaps. However, since the hierarchical policy here is also limited to the \emph{behavior primitives}, it cannot fully solve the task as illustrated in figure \ref{fig:transfer_hier_split}. In contrast, we consider a hierarchical policy with a \emph{separate} lower level controller for the policy (as in figure \ref{fig:structured_priors_descr}c) using the full KL reward between both priors from equation \ref{eq:objective:hierarchical} for training. As figure \ref{fig:transfer_hier_split} shows, this setup performs better on this task since the lower level controller can adapt and learn new behaviors corresponding to jumping. Interestingly we did not find a large gain from initializing the weights for the lower level posterior from the prior in this case indicating that there isn't much advantage of partial parameter sharing in this task.
%All of the experiments considered thus far share the lower level policy between the \bp and the policy.
%We consider an example task as shown in figure \ref{fig:transfer_hier_split} where the transfer domain requires \textit{new skills}. 
% In our example, we train a controller on the \textit{Locomotion (Ant)} task but transfer it to the \textit{Locomotion (Gaps)} task. The transfer domain consists of a room with a gap of variable length in the center of it. The agent is rewarded for moving forward at each time step but must learn to jump across larger gaps to consistently solve the task. In this example, the \textit{prior} with a shared lower level does not capture the behaviors required to solve the task optimally. As shown in figure \ref{fig:transfer_hier_split}, we can adapt the skills of the \bp into a new lower level policy using the model described in section \ref{sec:hier_experiments}.
\begin{figure}%
    \centering
    \includegraphics[scale=0.3]{figures/set_2/transfer_split.png}
    \caption{\textbf{Skill adaptation for hierarchical models} using separate lower level controllers on the \textit{Locomotion (Gap)} task.}
    \label{fig:transfer_hier_split}
    % \begin{subfigure}{0.5\textwidth}
    % \centering
\end{figure}

==> older_version/introduction.tex <==

\section{Introduction}
\label{sec:intro}

% Ideas:
% - prior knowledge over trajectories
% - different levels: highly-specific, smoothness, some features shared across different tasks, ...
% - modeling temporally extended, goal directed, and simple behavior
% - decouple statistics of behavior from model structure; but model structure can help
% 
% - connection to information theoretic regularization
% - connection to hierarchy
%
% 1. Advances but still challenging
% 2. Inject, extract, transfer knowledge
% 3. Probabilistic framework, model of trajectories, flexible
% 4. Allows us to express & learn prior knowledge, different levels of specificity & abstraction
% 5. Discuss the relation behavior statistics and model structure; discuss relationship to HRL
% 6. connection to information theoretic regularization

% \dhruva{Using the exploiting hierarchy paper to get things started for now.. rephrase and tweak later.}
Recent advances have greatly improved data efficiency, scalability, and stability of reinforcement learning  (RL) algorithms leading to successful applications in a number of domains ~\citep{heess2017emergence,riedmiller2018learning,andrychowicz2018learning,mnih2015human,OpenAI_dota,silver2016mastering}. 
%
%~\cite{rennie2017self,zoph2016neural,espeholt2018impala,ganin2018synthesizing,zhu2018dexterous}.
Many problems, however, still remain challenging to solve or require large numbers of interactions with the environment; a situation that is likely to get worse as we attempt to tackle increasingly challenging and diverse problems. One avenue for reducing sample complexity focuses on methods that learn behaviors that are shared across a range of tasks. For example, \citet{teh2017distral} show one way of how knowledge can be extracted across tasks in order to generalize to new ones. 

In this work, we approach this multi task learning problem through the lens of probabilistic modeling. Policies, when combined with the environment dynamics, define a distribution over trajectories. 
% We begin with the intuition that policies, combined with the environment dynamics, can be thought of as defining a distribution over trajectories.
Reasoning about policies in this way allows us to borrow tools and ideas from the rich literature on probabilistic modeling to arrive at a general framework for learning and using \textit{priors} in multi-task RL. We demonstrate how such priors can be used to capture useful \textit{behaviors} that are common across a range of tasks.
This can then be used to bootstrap learning on new tasks by constraining the space of trajectories generated for exploration. We describe how our framework can be extended to modular or hierarchical structures which can then be used to selectively constrain, transfer and generalize certain aspects of the behavior such as lower-level skills or high-level goals.


% A general avenue for reducing sample complexity in machine learning is the use of appropriate prior knowledge, or inductive biases. In RL, curricula, learning and transfer across task distributions, and the use of demonstrations have been shown to be powerful tools in this regard. 
% The success of these ideas, and more generally our ability to build agents that have a chance of succeeding in lifelong learning scenarios, relies on the ability to transfer and generalize behaviours across tasks, and thus on mechanisms for extracting knowledge from existing solutions and for using such knowledge to shape the solutions to new problems. 

% Recently \cite{teh2017distral,galashov2018information} have introduced a framework for knowledge representation and transfer in RL that allows to express and exploit inductive biases in reinforcement learning problems.
% The approach relies on a connection between the KL-regularized objective~\cite{todorov2007linearly,kappen2012optimal,rawlik2012stochastic,schulman2017equivalence} and probabilistic models. 
% One way to think of a policy is that, together with the environment dynamics, it defines a distribution over trajectories, and the framework uses probabilistic models of trajectories to express prior knowledge about the solution distribution of a RL problem. 
% To this end it introduces a second component, a \bp  to which the policy is encouraged to remain close in terms of the Kullback-Leibler (KL) divergence. This prior can simplify the learning problem, for instance by reducing the trajectory space that needs to be searched, or by steering the learning algorithm away from undesirable solutions. In this work, we expand on these intuitions to develop a more general framework that allows us to express richer, structured \bps  within the RL objective.

% Rather than manually crafting specific constraints which may or may not be appropriate for a given task or task distribution, it is possible to learn the prior from data, and \cite{teh2017distral,galashov2018information} have shown that this can be effective both in multi-task and transfer learning scenarios. \cite{galashov2018information} demonstrate how information asymmetry, i.e.\ restricting the prior's access to certain parts of the state space can be used to selectively transfer or generalize certain aspects of a learned behavior across tasks or different parts of the state space. In this work we expand on this intuition and show its application to structured or hierarchical \bps. 
% The hierarchical formulation gives rise to a modular structure that allows to selectively constrain, transfer and generalize certain aspects of the behavior, such as low-level skills or high-level goals. Exploiting the compositionality of probabilistic models, this modularity also facilitates the immediate reuse of some model components in a principled manner, such as the sharing of low-level skills across tasks. This allows imposing more flexible constraints and can reduce the number of model parameters leading to an increased statistical efficiency and faster learning.


% In this work, we explore two key intuitions related to \bp s:
The key insights that we develop in the rest of this work are as follows :
\begin{itemize}
    \item \textbf{\textit{Behavioral Priors} model trajectory distributions}: We develop the intuition of \bps as \textit{distributions over trajectories} that can be used to guide exploration and constrain the space of solutions. In this view, a good \bp is one that is general enough to capture the solutions to many tasks of interest while also being restrictive enough for tractable exploration.
    \item \textbf{Information regularization can induce generalization}:  We demonstrate that an information bottleneck can be used to learn \textit{priors} that can generalize across the trajectory space and empirically show that this can lead to faster learning.
    \item \textbf{Structure in the \bp model }: We develop a general framework that supports learning \bp models that can be structured into multiple hierarchical layers. We combine this intuition with an information bottleneck to demonstrate a method that learns to dissociate higher level goals from lower level behaviors.
\end{itemize}

The rest of this work is split into two main parts. First, in sections \ref{sec:BP} and \ref{sec:experiments} we introduce our method and conduct an initial set of experiments for analysis and ablation to help ground these ideas. Following that, we extend our method to learn structured models in section \ref{sec:structured_models}. In section \ref{sec:hier_experiments}, we then conduct a range of experiments that demonstrate how structured and unstructured \bps can be used to speedup learning and transfer behaviors to new tasks. Finally we discuss connections to related work in section \ref{sec:related} and conclude with section \ref{sec:conclusion}.

% The main contributions of this work are as follows :\\
% \begin{itemize}
%     \item Introduces a framework that shows how structured behavioral priors can be learned and used in RL.
%     \item Empirically demonstrates how behavioral priors can be used to regularize RL agents on new tasks.
%     \item Demonstrates that structured priors can model behavior at different levels of abstraction in a composable way. 
    
% \end{itemize}

% Structure:
%   Lot of success with RL etc. Ideas for options as well to capture interesting structure in the world. 
%   Recent focus on RL as inference (soft-Q, berkeley lab etc) has shown success. This work - Introduces notion of *priors* which has so far been ignored. Also describe that *options* or hierarchical structure can be incorporated into this. 
%   Describe subsections that will follow.

% ----------
%Backup

% \section{Introduction}
% \label{sec:intro}

% % \dhruva{Using the exploiting hierarchy paper to get things started for now.. rephrase and tweak later.}
% Recent advances have greatly improved data efficiency, scalability, and stability of reinforcement learning  (RL) algorithms leading to successful applications in a number of domains ~\cite{heess2017emergence,riedmiller2018learning,andrychowicz2018learning,mnih2015human,OpenAI_dota,silver2016mastering}. 
% %
% %~\cite{rennie2017self,zoph2016neural,espeholt2018impala,ganin2018synthesizing,zhu2018dexterous}.
% Many problems, however, still remain challenging to solve or require large numbers of interactions with the environment; a situation that is likely to get worse as we attempt to tackle increasingly challenging and diverse problems. One avenue for reducing sample complexity focuses on methods that learn behaviors that are shared across a range of tasks. For example, [TODO: Cite distral etc] show one way of how knowledge can be extracted across tasks in order to generalize to new ones. \dhruva{Maybe mention meta world and the community thinking about designing multi-task suites. Or are we shooting ourselves in the foot by talking about it?}

% In this work however, we approach the multi task learning problem through the lens of probabilistic modeling. We begin with the intuition that policies, combined with the environment dynamics, can be thought of as defining a distribution over trajectories. We develop on this idea by borrowing tools from the probabilistic modeling literature to arrive at a general framework for learning \textit{priors} in multi-task RL.  Our approach models priors that can be used to capture a general set of \textit{behaviors} that are common across a range of tasks. These \bps  can then be used to bootstrap learning on new tasks by constraining the space of trajectories generated for exploration. Using this framework we model structured or hierarchical \bps  where a modular structure can be used to selectively constrain, transfer and generalize certain aspects of the behavior such as lower-level skills or high-level goals.


% % A general avenue for reducing sample complexity in machine learning is the use of appropriate prior knowledge, or inductive biases. In RL, curricula, learning and transfer across task distributions, and the use of demonstrations have been shown to be powerful tools in this regard. 
% % The success of these ideas, and more generally our ability to build agents that have a chance of succeeding in lifelong learning scenarios, relies on the ability to transfer and generalize behaviours across tasks, and thus on mechanisms for extracting knowledge from existing solutions and for using such knowledge to shape the solutions to new problems. 

% % Recently \cite{teh2017distral,galashov2018information} have introduced a framework for knowledge representation and transfer in RL that allows to express and exploit inductive biases in reinforcement learning problems.
% % The approach relies on a connection between the KL-regularized objective~\cite{todorov2007linearly,kappen2012optimal,rawlik2012stochastic,schulman2017equivalence} and probabilistic models. 
% % One way to think of a policy is that, together with the environment dynamics, it defines a distribution over trajectories, and the framework uses probabilistic models of trajectories to express prior knowledge about the solution distribution of a RL problem. 
% % To this end it introduces a second component, a \bp  to which the policy is encouraged to remain close in terms of the Kullback-Leibler (KL) divergence. This prior can simplify the learning problem, for instance by reducing the trajectory space that needs to be searched, or by steering the learning algorithm away from undesirable solutions. In this work, we expand on these intuitions to develop a more general framework that allows us to express richer, structured \bps  within the RL objective.

% % Rather than manually crafting specific constraints which may or may not be appropriate for a given task or task distribution, it is possible to learn the prior from data, and \cite{teh2017distral,galashov2018information} have shown that this can be effective both in multi-task and transfer learning scenarios. \cite{galashov2018information} demonstrate how information asymmetry, i.e.\ restricting the prior's access to certain parts of the state space can be used to selectively transfer or generalize certain aspects of a learned behavior across tasks or different parts of the state space. In this work we expand on this intuition and show its application to structured or hierarchical \bps. 
% % The hierarchical formulation gives rise to a modular structure that allows to selectively constrain, transfer and generalize certain aspects of the behavior, such as low-level skills or high-level goals. Exploiting the compositionality of probabilistic models, this modularity also facilitates the immediate reuse of some model components in a principled manner, such as the sharing of low-level skills across tasks. This allows imposing more flexible constraints and can reduce the number of model parameters leading to an increased statistical efficiency and faster learning.


% % In this work, we explore two key intuitions related to \bp s:
% The key insights that we develop in the rest of this work are as follows :
% \begin{itemize}
%     \item \textbf{\textit{Behavioral Priors} model trajectory distributions}: We develop the intuition of \bp s as \textit{distributions over trajectories} that can be used to guide exploration. In this view, a good \bp is one that is general enough to capture the solutions to many tasks of interest while also being restrictive enough for tractable exploration.
%     \item \textbf{Structure in the \bp model }: We develop a general framework that supports learning \bp models that can be structured into multiple hierarchical layers. We also conduct an experimental analysis with various models that demonstrate how \bps can be used to capture long term temporal correlations with complex bodies and thus speed up learning on difficult tasks.
%     % We show how structured or hierarchical \bp s can capture different levels of complexity in each sub-component. We demonstrate how this property can be exploited to solve complex tasks by simply re-combining these sub-components in novel ways.
%     \item \textbf{Information regularization can induce generalization}: A final key aspect that we explore is to show how restricting certain information can lead to policies that generalize across the trajectory space. We show experimentally how this leads to a natural way of modeling structured \bps. 
% \end{itemize}

% The remainder of the text is organized as follows \dhruva{Update this to indicate the new structure i.e. two sets of experiments.}
% % The main contributions of this work are as follows :\\
% % \begin{itemize}
% %     \item Introduces a framework that shows how structured behavioral priors can be learned and used in RL.
% %     \item Empirically demonstrates how behavioral priors can be used to regularize RL agents on new tasks.
% %     \item Demonstrates that structured priors can model behavior at different levels of abstraction in a composable way. 
    
% % \end{itemize}

% % Structure:
% %   Lot of success with RL etc. Ideas for options as well to capture interesting structure in the world. 
% %   Recent focus on RL as inference (soft-Q, berkeley lab etc) has shown success. This work - Introduces notion of *priors* which has so far been ignored. Also describe that *options* or hierarchical structure can be incorporated into this. 
% %   Describe subsections that will follow.

==> older_version/learning_priors.tex <==
\section{Behavioral Priors for Control}
\label{sec:BP}

We now introduce a method that allows us to express prior knowledge about solution trajectories in RL. We begin by considering the KL-regularized RL formulation \citep{todorov2007linearly,kappen2012optimal,rawlik2012stochastic,schulman2017equivalence}: 

\begin{align}
\mathcal{L}
&= \EE_\qp[ \sum_t r(s_t,a_t)] - 
\KL[ \qp(\tau) || \pp(\tau) ]. \label{eq:objective:generic}
\end{align}
where $r_t$ is the instantaneous reward at time $t$ and 'KL' refers to the Kullback Leibler divergence between the two distributions.

This objective trades off maximizing returns with staying close (in the KL sense) to some reference behavior: $\pp$. Broadly speaking we can classify existing approaches that make use of this objective into two categories based on the choice of $\pp$. One approach, simply sets $\pp$ to be a uniform distribution over actions resulting in the entropy-regularized objective as used by ~\citet{ziebart2010modeling,schulman2017equivalence,haarnoja2017reinforcement,haarnoja2018soft,hausman2018learning}. While this approach has been motivated in many ways, it has been shown to be helpful in - preventing the policy from collapsing to a deterministic solution; improving exploration; and increasing the robustness of the policy to perturbations in the environment. 
%
A second class of algorithms optimize $\mathcal{L}$ with respect to both $\qp$ and $\pp$ and are often referred to as \emph{EM-policy search} algorithms. Examples of this style of algorithms include \citet{Peters10,toussaint2006probabilistic,rawlik2012stochastic,levine2013variational,levine2016end,montgomery2016guided,chebotar2016path,abdolmaleki2018maximum}. In each of these approaches the specific forms for $\qp$ and $\pp$ can lead to differences in the optimization scheme. Generally speaking, here $\pp$ plays the role of a trust-region that limits the change in $\qp$ on each iteration but does not constrain the final solution. 

In this work, we focus on a different formulation that seeks to cast $\pp$ as a \bp. That is, we seek a form of $\pp$ that can model more sophisticated behaviors that can lead to good final solutions. In our view, $\pp$ can be thought of as a regularizer that, much like a shaping reward, can guide the learning process. In what follows, we present an approach that can \textit{learn} $\pp$ from data by generalizing the approach considered by ~\citet{teh2017distral}.

% The intuition behind our approach is to force $\pp$ to model a more general 
% \dhruva{Include Nicolas' visualization of trajectory spaces here?}

% In this case the KL regularized setup allows us to express the desire that we want to learn solutions in which much of the behavior can be shared across tasks, i.e.\ that there is significant overlap between the trajectory distributions for different tasks.
% This can be formalized as follows:
We begin by considering the multi-task RL setting as in ~\citet{teh2017distral}:
\begin{align}
% &= \log \sum_k p(k) \int p(\tau) p(R=1|\tau, k) d\tau \\
\mathcal{L} = \sum_w p(w) \EE_{\qp_w} [ \sum_t r_w(s_t,a_t)] - \KL[ \qp_w(\tau) || \pp(\tau) ], 
\label{eq:ProbabilisticRL:MultitaskKL}
\end{align}
where $p(w)$ is some distribution over tasks, the reward function is a function of the task $w$, and the policy $\qp_w(\tau)$ has knowledge of the task, while the prior $\pp(\tau)$ does not.
%
Here, we have that the  optimal policy $\qp_w$ and prior $\pp$ are given by:
\begin{align}
\qp^*_w( a | s_t) =  \pp(a_t|s_t)\exp(Q^*_w(s_t,a) - V^*_w(s_t)),
\label{eq:ProbabilisticRL:OptimalExpert}
\end{align}
and
\begin{align}
\pp^* &= \arg \min_{\pp} \sum_w p(w) \EE_{x_t \sim d_{\qp_{w,t}} } [ \KL [ \qp_w(\cdot | x_t) || \pp(\cdot | x_t) ]]\\
&= \arg \max_{\pp} \sum_w p(w) \EE_{x_t \sim d_{\qp_{w,t}} } [ \EE_{\qp_w(\cdot | x_t)}[ \log \pp(\cdot | x_t) ]]\\
&= \sum_w p(w|x_t) \qp_{w}(a_t | x_t) \label{eq:ProbabilisticRL:OptimalPrior}
\end{align}

In other words the optimal prior $\pp^*$ can be viewed as a \textit{weighted mixture} of the task specific policies that can be trained via supervised learning. Note that if $\pp$ had access to all the information of $\qp$, then the optimal solution would be to just set $\pp^*=\qp^*$. Thus, restricting the information that $\pp$ has access to results in a more \emph{general} policy that spans a broader space of solutions to many tasks. 
%
% while the optimal task solution $\qp^*_w$ is achieved by \textit{re-weighting} $\pp$ with the exponentiated Q function. 
In this work, we generalize this intuition by considering  priors $\pp$ which are \textit{restricted} by limiting their modeling capacity or the information they have access to. Such priors would be forced to learn general behaviors that are common across different settings of the unmodeled or inaccessible parts of the state space.% which would be more generally applicable across different tasks. 
% To make this intuition more concrete, consider an example scenario where an agent must move boxes to specific goal locations. A prior that does not see the goals would still learn behaviors related to moving boxes around in the world. 

Our method for training \bps can be easily incorporated into any RL method. For this work, we adapt the off-policy SVG-0 algorithm \citep{heess2015learning} using the retrace estimator \citep{munos2016safe} as shown in algorithm \ref{alg:rs0_distral}. 

% In this case, the specific \textit{task} is hidden from the prior forcing it to \textit{generalize} to match distributions generated by $\qp$. Note that there may be other approaches to regularization that can have a similar generalization effect - the point here is mainly that controlling information flow is a natural, and relatively unexplored way to do this in a multi-task regime. Another point to note here is that in general one may make different choices for information that is be withheld from the \bp. This results in a trade-off between its ability to generalize on the one hand and its usefulness for exploration on a particular task on the other. We explore this aspect in greater detail in section \ref{sec:experiments}.

\begin{algorithm*}[tb]
  \caption{Learning \textit{priors}: SVG(0)~\citet{heess2015learning} with experience replay}
  \label{alg:rs0_distral}
\begin{algorithmic}
  \State Policy: $\pi_\theta(a_t|x_t)$ with parameter $\theta$
  \State \textit{Behavioral Priors}: $\pi_{0,\phi}(z_t|x_t)$
  \State Q-function: $Q_\psi(a_t, x_t)$ with parameter $\psi$
  \State Initialize target parameters $\theta^\prime \leftarrow \theta$,
  \hspace{0.2cm} $\phi^\prime \leftarrow \phi$, \hspace{0.2cm} $\psi^\prime \leftarrow \psi$.
  \State Target update counter: $c \leftarrow 0$
  \State Target update period: $P$
  \State Replay buffer: $\mathcal{B}$
  \Repeat
  \For{$j=0, 1, 2, ... $}
  \State Sample partial trajectory $\tau_{t:t+K}$ with action log likelihood $l_{t:t+K}$ from replay $\mathcal{B}$:\\ \hspace{1.6cm}$\tau_{t:t+K}=(s_t,a_t,r_t,...,r_{t+K})$,\\
  \hspace{1.6cm}$l_{t:t+K}=(l_t,...,l_{t+K})=(\log\mu(a_t|x_t),...,\log\mu(a_{t+K}|x_{t+K}))$
  %\STATE Compute KL: $\hat{\KL}_{t^\prime}=\KL\left(z|x_{t^\prime}\right)+\KL\left(a|z_{t^\prime},x_{t^\prime}\right)$
  \State Compute KL:\\
  \hspace{1.6cm}$\hat{\KL}_{t^\prime}=\KL\left[\pi_\theta(.|x_{t^\prime})\|\pi_{0,{\phi^\prime}}(.|x_{t^\prime})\right]$
  \State Compute KL for Distillation:\\
  \hspace{1.6cm}$\hat{\KL}^\mathcal{D}_{t^\prime}=\KL\left[\pi_\theta(.|x_{t^\prime})\|\pi_{0,{\phi}}(.|x_{t^\prime})\right]$
  \State Compute action entropy:
  $\hat{\text{H}}_{t^\prime}=\EE_{\pi_\theta(a|x_{t^\prime})}[\log\pi_\theta(a|x_{t^\prime})]$
  \State Estimate bootstrap value:
  $\hat{V}_{t^\prime}
        =\EE_{\pi_\theta(a|x_{t^\prime})}
        \left[Q_{\psi^\prime}(a,x_{t+K})\right]-\alpha\hat{\KL}_{t+K}$
  \State Estimate traces~\citet{munos2016safe}:
  $\hat{c}_{t^\prime}=\lambda \min\left(\frac{\pi_\theta(a_{t^\prime}|,x_{t^\prime})}{l_{t^\prime}}\right)$
  \State Apply Retrace to estimate Q targets~\citet{munos2016safe}:\\
  \hspace{1.6cm}
  $\hat{Q}^R_{t^\prime}=Q_{\psi^\prime}(a_{t^\prime},x_{t^\prime})
        +
        \sum_{s \ge t^\prime}\gamma^{s-t^\prime}\left(\prod_{i=s}^{t^\prime}\hat{c}_i\right)
        \left(r_s+\gamma\left(\hat{V}_{s+1}-\alpha\hat{\KL}_{s+1}\right)Q_{\psi^\prime}(a_s,x_s)\right)$
  \State Policy loss: $\hat{L}_\pi=\sum_{i=t}^{t+K-1}\EE_{\pi_\theta(a|\epsilon_{i},x_{i})}Q_{\psi^\prime}(a,x_{i})-\alpha\hat{\KL}_i + \alpha_\text{H}\hat{\text{H}}_i$
  \State Q-value loss: $\hat{L}_Q=\sum_{i=t}^{t+K-1}\|\hat{Q}^R_i-Q_\psi(a,x_{i})\|^2$
  \State \textit{Behavioral Prior} loss: $\hat{L}_{\pi^H_0}=\sum_{i=t}^{t+K-1}\hat{KL}_i^\mathcal{D}$
  \State
  $\theta \leftarrow \theta+\beta_\pi\nabla_\theta\hat{L}_\pi$ \hspace{0.3cm}
  $\phi \leftarrow \phi+\beta_{\pi}\nabla_\phi\hat{L}_{\pi}$
  \hspace{0.3cm}
  $\psi \leftarrow \psi-\beta_{Q}\nabla_\psi\hat{L}_{Q}$
  \State Increment counter $c \leftarrow c+1$
  \If{$c > P$}
  \State Update target parameters $\theta^\prime \leftarrow \theta$,
  \hspace{0.2cm} $\phi^\prime \leftarrow \phi$, \hspace{0.2cm} $\psi^\prime \leftarrow \psi$
  \State $c \leftarrow 0$
  \EndIf
  \EndFor
  \Until
\end{algorithmic}
\end{algorithm*}

% % 1. "Learning" the prior. \\

% % Structure:
%     % Start with the equations for RL as inference with the prior policy for a distribution over tasks. Can refer to Nicolas' tech report for a more detailed summary. Importance of information asymmetry and how it allows the generalization to take place. Highlight how this can be viewed as distributions over trajectories i.e. the main policy specializes in a subspace of trajectories while the default policy can cover more of the trajectory space and hence generalize (to new tasks) better.



% So far, we only briefly mentioned the general term $p(R=1|\tau)$ that measures the compatibility between the trajectories and a pseudo-observation of optimality $R=1$.
% Choosing:
% \begin{align}
% \log p(R=1|\tau) & = \sum_t r(s_t,a_t) 
% \label{eq:objective:reward}
% \end{align}
% we can recover a regularized form of the expected reward objective, similar to the one introduced in Sec.~\ref{sec:KL-RL}, which is a generalization of the one commonly used in the RL literature:

% To start with consider the problem of evaluating the following quantity:
% \begin{align}
% L = \log \int \pp(\tau) p(R=1|\tau) d\tau.
% \label{eq:log_marginal_likelihood}
% \end{align}
% where $\pp(\tau)$  is a distribution over trajectories. We can think of the pseudo-observation $R=1$ as an optimality indicator. In other words it measures the compatibility of a trajectory with some notion of optimality.
%  Evaluating $L$ in equation (\ref{eq:log_marginal_likelihood}) can then be seen as an inference problem. Using Jensen's inequality introduced in Section \ref{sec:ELBO}, we can lower bound $L$ by introducing a distribution $\qp(\tau)$ over trajectories as follows:
% \begin{align}
% L = \log \int \pp(\tau) p(R=1|\tau) d\tau &= \log \EE_\qp \frac{\pp(\tau) p(R=1|\tau)}{\qp(\tau)} d\tau \\
% &\geq 
% \int \qp(\tau) \log 
% \frac{\pp(\tau) p(R=1|\tau)}{\qp(\tau)} d\tau \\
% &= \int \qp(\tau) \log p(R=1|\tau) d\tau +
% \int \qp(\tau)\log \frac{\pp(\tau)}{\qp(\tau)} d\tau\\
% &=\EE_\qp[ \log p(R=1|\tau) ] - \KL[ \qp || \pp]. %\\
% % &=L - \KL[ q(\Tau) || p(\Tau | R=1) ].
% \end{align}


==> older_version/structured_priors.tex <==
\section{Structured \bp models}
\label{sec:structured_models}

In this section we expand on the ideas introduced in section \ref{sec:BP} to consider richer forms of $\pp$ and $\qp$ that contain latent variables. Latent variable models are a common tool in probabilistic modeling to increase capacity, introduce inductive biases, learn useful representations and model complex distributions. Additionally the use of latent variables in the policy may lead to modular representations of behavior. While latent variables hold much promise, a number of modelling choices and practical decisions stem from having to tractably compute or approximate the KL term in equation \ref{eq:objective:generic}: $\KL[ \qp(\tau) || \pp(\tau) ]$. We outline a general framework describing this in detail below.

For both the $\pp$ and for $\qp$, we can consider general directed latent variable models of the following form:
\begin{align}
\pp(\tau) &= \textstyle \int \pp(\tau| y) \pp(y) d y,\\
\qq(\tau) &= \textstyle \int \qq(\tau | z) \qq(z) d z
\end{align}
where both $y$ and $z$ can be time varying, e.g.\ $y=(y_1, \dots y_T)$, continuous or discrete, and can exhibit further structure (and thus include e.g.~binary variables that model option termination). This form can be convenient when $\pp(a_t | x_t)$ and $\qp(a_t | x_t)$ are tractable (when $z$ or $y$ have a small number of discrete states or decompose conveniently over time as in \citet{fox2017multi,krishnan2017discovery}).

In general, however, latent variables in $\pp$ and $\qq$ may introduce the need for additional approximations. To start with, consider the case where only $\pp$ contains latent variables. This results in the following lower bound to $\mathcal{L}$:
\begin{align}
\mathcal{L} 
&= \textstyle \EE_\qp[ \sum_t r(s_t,a_t)] - 
\KL[ \qp(\tau) || \pp(\tau) ]\\
&\geq \textstyle \EE_\qp \left [ \sum_t r(s_t,a_t) + \EE_f \left [ \log\frac{\pp(\tau,y)}{f(y|\tau)} \right ] \right] + \Ent [ \qp(\tau) ]\\
&= \textstyle \EE_\qp\left [ \sum_t r(s_t,a_t) + \EE_f \left [ \log \pp(\tau|y) \right ] \right. \nonumber\\
&\hspace{1.8cm}-\left. \KL [ f(y|\tau) || \pp(y) ] \right] + \Ent [ \qp(\tau) ]. \label{eq:objective:prior_ELBO}
\end{align}
If $y_t$ are discrete and take on a small number of values we can compute $f(y|\tau)$ exactly (e.g.~using the forward-backward algorithm as in \cite{fox2017multi,krishnan2017discovery}); in other cases we can learn a parameterized approximation to the true posterior or can conceivably apply mixed inference schemes \citep[e.g.][]{johnson2016composing}.


On the other hand, if only $\qp$ contains latent variables $z_t$ which could be continuous, this results in an alternative approximation as discussed in \cite{hausman2018learning}:
\begin{align}
\mathcal{L} &= \EE_\qp[\sum_t r(x_t, a_t) ] 
- \EE_\qp [ \KL[ \qp(\tau) || \pp(\tau) ] ] \\
&\geq 
\EE_\qp[\sum_t r(x_t, a_t) ] 
+ \EE_\qp \left [ \log \frac{\pp(\tau)g(z | \tau)}{\qp(\tau | Z)\qp(Z) } \right ]
\label{eq:objective:posterior_bound_1}
\\
&= \EE_\qp[\sum_t r(x_t, a_t) ] 
+ \EE_\qp \left [ \log \pp(\tau) + \log g(z | \tau) \right ] + \Ent [ \qp(\tau | Z) ] + \Ent [\qp(Z) ]
\label{eq:objective:posterior_bound_full}
\end{align}
where $g$ is a learned approximation to the true posterior $\qq(z|\tau)$. 
%
This general expression can be specialized to suit different modelling needs. It allows modelling per-timestep multimodality in the action space as well as temporal correlations over time. For instance, \cite{hausman2018learning} considers the special case when $z$ is sampled once a the beginning of the episode. This formulation bears interesting similarities with diversity inducing regularization schemes based on mutual information \citep[e.g.][]{gregor2016variational,florensa2017stochastic} but arises here as an approximation to trajectory entropy. This formulation also has interesting connections to auxiliary variable formulations in the approximate inference literature \cite{salimans2014bridging,agakov2004an}. An alternative approach is considered by \cite{haarnoja2018latent} who consider a parametric form for policies with latent variables for which the entropy term can be computed analytically and no approximation is needed.

In this work, we consider a formulation with latent variables in \emph{both} $\pp$ and $\qp$. For simplicity and concreteness, we consider a continuous the latent variable $z_t$ which has the same dimension and semantics in $\qq$ and $\pp$. We divide $\qp$ into higher level (HL) $\qp^H(z_t| x_t)$ and lower level (LL)  $\qp^L(a_t| z_t, x_t)$ components. We can then derive the following bound for the KL:
\begin{align}
\KL[\qp(a_t|x_t) || \pp(a_t|x_t)]
\le& \KL[\qp(a_t|x_t) || \pp(a_t|x_t)] + \EE_{\qp(a_t|x_t)}[\KL[\qp^H(z_t|x_t) || \pp^H(z_t|x_t)]] \nonumber \\
=&
\EE_{\qp(a_t|x_t)}[
\textstyle \log \frac{\qp(a_t|x_t)}{\pp(a_t|x_t)}] \nonumber\\
 &\textstyle +\EE_{\qp(a_t|x_t)}[
\EE_{\qp^H(z_t|a_t,x_t)}[\textstyle \log \frac{\qp^H(z_t|a_t,x_t)}{\pp^H(z_t|a_t,x_t)}]
\nonumber \\
=&
\EE_{\qp(a_t,z_t|x_t)}[
\textstyle \log \frac{\qp(a_t,z_t|x_t)}{\pp(a_t,z_t|x_t)}]
%\nonumber \\ 
=%& 
\KL(z_t,a_t|x_t) \nonumber \\
=&
\EE_{\qp^H(z_t|x_t)}[
\textstyle \log \frac{\qp^H(z_t|x_t)}{\pp^H(z_t|x_t)}] \nonumber \\
 &\textstyle +\EE_{\qp^H(z_t|x_t)}[
\EE_{\qp^L(a_t|z_t,x_t)}[\textstyle \log \frac{\qp^L(a_t|z_t,x_t)}{\pp^L(a_t|z_t,x_t)}]
\nonumber \\
=&\KL[\qp^H(z_t|x_t) || \pp^H(z_t|x_t)]  + \EE_{\qp^H(z_t|x_t)}[\KL[\qp^L(a_t|z_t, x_t) || \pp^L(a_t|z_t, x_t)] ]
\label{eq:objective:hierarchical}
\end{align}
which can be approximated via Monte Carlo sampling and $\tau$ is a trajectory that contains $z_t$s.

\subsection{Practical considerations}
In the remainder of this section, we describe some practical considerations that are needed in order to implement the KL-regularized objective using equation \ref{eq:objective:hierarchical}.

\paragraph{Regularizing using information asymmetry} 
As discussed in section \ref{sec:BP} and illustrated in section \ref{sec:experiments}, information asymmetry can be a powerful tool for generalization and regularizing behaviors. We can extend this intuition to the hierarchical setting and introduce an asymmetry between the information processed by the higher ($\qp^H$) and lower level ($\qp^L$) policy. Varying the information sent to each level allows the lower level to learn task-agnostic behaviors and creates a separation of roles between $\qp^H$ and $\qp^L$. Similarly, we hide task specific information from both $\pp^L$ and $\pp^H$, which in turn makes the marginal default policy $\pp$ to be agnostic to the task.

\paragraph{Partial parameter sharing}
\label{sec:hierarchy:sharing}
An advantage of the hierarchical structure of the policies is that it enables several options for partial parameter sharing, which when used in the appropriate context can make learning more statistically efficient. We explore the utility of sharing low-level controllers between agent and default policy, i.e.\ $\qp^L(a_t|z_t,x_t)=\pp^L(a_t|z_t,x_t)$, and study the associated trade-offs in different learning scenarios. This simplifies the training objective from equation \ref{eq:objective:hierarchical} to:

\begin{align}
\mathcal{L}(\qp, \pp) & \textstyle \geq \textstyle \EE_{\tau}\left[
\sum_{t\ge1} \gamma^t r(s_t,a_t)
    - \alpha\gamma^t\KL[\qp(z_t | x_t) || \pp(z_t | x_t)] \right]
    \label{eq:latent_lower_bound}
\end{align}

where the KL divergence is between policies defined on abstract actions $z_t$ only. We illustrate the various approaches to training structured and unstructured models with shared and separate lower levels in figure \ref{fig:structured_priors_descr}.
\dhruva{At this point we can discuss Goyal et al but maybe leave this discussion to related work.}
%
\begin{figure}%
    \centering
    \includegraphics[height=6cm]{figures/set_2/structure_information_asymmetry.png}
    \caption{\textbf{Training setup for structured and unstructured models.}}
    \label{fig:structured_priors_descr}
\end{figure}

\paragraph{Algorithmic considerations}
Similar to \cite{heess2016learning}, we reparameterize $z_t\sim \pi^H(z_t|x_t)$ as $z_t = f^H(x_t, \epsilon_t)$, where 
$\epsilon_t \sim \rho(\epsilon_t)$ is a fixed noise distribution and
$f^H(\cdot)$ is a deterministic function. 
In practice this means that the hierarchical policy can be treated as a flat policy $\pi(a_t|\epsilon_t,x_t)=\pi^L(a_t|f^H(x_t, \epsilon_t), x_t)$ and can be optimized by backpropagating the gradient from an action value function $Q(a_t, z_t, x_t)$. Note that here the latent variable $z_t$ may be sampled infrequently. This requires extra care in terms of learning the action value function  $Q(a_t, z_t, x_t)$ in an off-policy setting. Specifically, we adapt the off-policy correction scheme introduced in \citet{munos2016safe} to include latent variables as described below:
\begin{equation}
\textstyle
\hat{Q}^R_{t}=Q_t
        +\sum_{s \ge t}\gamma^{s-t^\prime}\left(\prod_{i=s}^{t}c_i\right)
        \delta_sQ,
\end{equation}
where $\delta_sQ=r_s+\gamma(\hat{V}_{s+1}-\alpha\KL_{s+1})-Q_s$ and  $Q_t=Q(a_{t},z_{t},x_{t})$.
$\hat{V}_s=\EE_{\pi(a|\epsilon_t,x_t)}[Q(a,z_{t},x_{t})]$ is the estimated bootstrap value, $\KL_{s}=\KL\left[\pi^H(z|x_{s})\|\pi^H_{0}(z|x_{s})\right]+\KL\left[\pi^L(a|z_s,x_{s})\|\pp^L(a|z_s,x_{s})\right]$ and $\gamma$ is the discount.
$c_{i}=\lambda \min\left(\frac{\pi(a_{i}|\epsilon_{i},x_{i})}{\mu(a_i|x_i)}\right)$ is truncated importance weight called \textit{traces}.

With these changes we implement a hierarchical version of the off-policy algorithm SVG-0 introduced in \cite{heess2015learning} as shown in Algorithm \ref{alg:r2h2}.
% Mention:
% 0. Info asymmetry in hierarchial setting.
% 1. Reparameterization trick for z_t
% 2. Partial parameter sharing with figure.
% 3. Q learning with RETRACE and latent variables.
% 4. Algorithm (which may be moved).

% We begin by reintroducing equation \ref{eq:objective:generic}:

% \begin{align}
% \mathcal{L}
% &= \EE_\qp[ \sum_t r(s_t,a_t)] - 
% \KL[ \qp(\tau) || \pp(\tau) ]. \label{eq:objective:generic_copy}
% \end{align}
%
% We would like to augment this with policies where either $\qp$ or $\pp$ or both contain latent variables. For the rest of this work we focus on the case where we \textit{both} $\qp$ and $\pp$ contain a latent variable and defer the discussion of other cases to Appendix \ref{appendix:general_framework}.

\begin{algorithm*}[tb]
  \caption{SVG(0)~\citet{heess2015learning} with experience replay for hierarchical policy}
  \label{alg:r2h2}
\begin{algorithmic}
  \State Flat policy: $\pi_\theta(a_t|\epsilon_t,x_t)$ with parameter $\theta$
  \State HL policy: $\pi^H_\theta(z_t|x_t)$, where latent is sampled by reparameterization $z_t=f^H_\theta(x_t, \epsilon_t)$
  \State \textit{Behavioral Priors}: $\pi^H_{0,\phi}(z_t|x_t)$ and $\pi^L_{0,\phi}(a_t|z_t,x_t)$ with parameter $\phi$
  \State Q-function: $Q_\psi(a_t,z_t,x_t)$ with parameter $\psi$
  \State Initialize target parameters $\theta^\prime \leftarrow \theta$,
  \hspace{0.2cm} $\phi^\prime \leftarrow \phi$, \hspace{0.2cm} $\psi^\prime \leftarrow \psi$.
  \State Target update counter: $c \leftarrow 0$
  \State Target update period: $P$
  \State Replay buffer: $\mathcal{B}$
  \Repeat
  \For{$t=0, K, 2K, ... T$}
  \State Sample partial trajectory $\tau_{t:t+K}$ with action log likelihood $l_{t:t+K}$ from replay $\mathcal{B}$:\\ \hspace{1.6cm}$\tau_{t:t+K}=(s_t,a_t,r_t,...,r_{t+K})$,\\
  \hspace{1.6cm}$l_{t:t+K}=(l_t,...,l_{t+K})=(\log\mu(a_t|x_t),...,\log\mu(a_{t+K}|x_{t+K}))$
  \State Sample latent: $\epsilon_{t^\prime} \sim \rho(\epsilon)$, $z_{t^\prime}=f^H_\theta(x_{t^\prime},\epsilon_{t^\prime})$
  %\STATE Compute KL: $\hat{\KL}_{t^\prime}=\KL\left(z|x_{t^\prime}\right)+\KL\left(a|z_{t^\prime},x_{t^\prime}\right)$
  \State Compute KL:\\
  \hspace{1.6cm}$\hat{\KL}_{t^\prime}=\KL\left[\pi^H_\theta(z|x_{t^\prime})\|\pi^H_{0,{\phi^\prime}}(z|x_{t^\prime})\right]+
  \KL\left[\pi^L_\theta(a|z_{t^\prime},x_{t^\prime})\|\pi^L_{0,\phi^\prime}(a|z_{t^\prime},x_{t^\prime})\right]$
  \State Compute KL for Distillation:\\
  \hspace{1.6cm}$\hat{\KL}^\mathcal{D}_{t^\prime}=\KL\left[\pi^H_\theta(z|x_{t^\prime})\|\pi^H_{0,{\phi}}(z|x_{t^\prime})\right]+
  \KL\left[\pi^L_\theta(a|z_{t^\prime},x_{t^\prime})\|\pi^L_{0,\phi}(a|z_{t^\prime},x_{t^\prime})\right]$
  \State Compute action entropy:
  $\hat{\text{H}}_{t^\prime}=\EE_{\pi_\theta(a|\epsilon_{t^\prime},x_{t^\prime})}[\log\pi_\theta(a|\epsilon_{t^\prime},x_{t^\prime})]$
  \State Estimate bootstrap value:
  $\hat{V}_{t^\prime}
        =\EE_{\pi_\theta(a|\epsilon_{t^\prime},x_{t^\prime})}
        \left[Q_{\psi^\prime}(a,z_{t+K},x_{t+K})\right]-\alpha\hat{\KL}_{t+K}$
  \State Estimate traces~\citet{munos2016safe}:
  $\hat{c}_{t^\prime}=\lambda \min\left(\frac{\pi_\theta(a_{t^\prime}|\epsilon_{t^\prime},x_{t^\prime})}{l_{t^\prime}}\right)$
  \State Apply Retrace to estimate Q targets~\citet{munos2016safe}:\\
  \hspace{1.6cm}
  $\hat{Q}^R_{t^\prime}=Q_{\psi^\prime}(a_{t^\prime},z_{t^\prime},x_{t^\prime})
        +
        \sum_{s \ge t^\prime}\gamma^{s-t^\prime}\left(\prod_{i=s}^{t^\prime}\hat{c}_i\right)
        \left(r_s+\gamma\left(\hat{V}_{s+1}-\alpha\hat{\KL}_{s+1}\right)Q_{\psi^\prime}(a_s,z_s,x_s)\right)$
  \State Policy loss: $\hat{L}_\pi=\sum_{i=t}^{t+K-1}\EE_{\pi_\theta(a|\epsilon_{i},x_{i})}Q_{\psi^\prime}(a,z_{i},x_{i})-\alpha\hat{\KL}_i + \alpha_\text{H}\hat{\text{H}}_i$
  \State Q-value loss: $\hat{L}_Q=\sum_{i=t}^{t+K-1}\|\hat{Q}^R_i-Q_\psi(a,z_{i},x_{i})\|^2$
  \State \textit{Behavioral Prior} loss: $\hat{L}_{\pi^H_0}=\sum_{i=t}^{t+K-1}\hat{KL}_i^\mathcal{D}$
  \State
  $\theta \leftarrow \theta+\beta_\pi\nabla_\theta\hat{L}_\pi$ \hspace{0.3cm}
  $\phi \leftarrow \phi+\beta_{\pi^H_0}\nabla_\phi\hat{L}_{\pi^H_0}$
  \hspace{0.3cm}
  $\psi \leftarrow \psi-\beta_{Q}\nabla_\psi\hat{L}_{Q}$
  \State Increment counter $c \leftarrow c+1$
  \If{$c > P$}
  \State Update target parameters $\theta^\prime \leftarrow \theta$,
  \hspace{0.2cm} $\phi^\prime \leftarrow \phi$, \hspace{0.2cm} $\psi^\prime \leftarrow \psi$
  \State $c \leftarrow 0$
  \EndIf
  \EndFor
  \Until
\end{algorithmic}
\end{algorithm*}

% Given a restricted set of information, another choice that could affect the efficacy of a \bp is the underlying model used to capture the trajectory space. A common tool in probabilistic modeling is the use of latent variable models which can increase capacity, introduce inductive biases that improve exploration and enable learning of useful representations. From an RL perspective this flavor of models are usually studied in the hierarchical RL (HRL) literature.

% We can augment the general expression in \ref{eq:objective:generic} with the introduction of a latent variable to either $\qp$ or $\pp$ or both. Here, we focus on the case where both have latent variables and leave the more general discussion to Appendix \ref{appendix:general_framework}.

% For concreteness, but without loss of generality, let $z_t$ be a (continuous) latent variable for each time step $t$ (we discuss alternative choices such as latent variables that are sampled infrequently in Appendices~\ref{appendix:general_framework}~and~\ref{appendix:derivations}). The agent policy is extended as $\qq(a_t,z_t|s_t)= \qq^H(z_t|s_t)\qq^L(a_t|z_t,s_t)$ and likewise for the default policy $\pp$.  $z_t$ can be interpreted as a high-level or abstract action, taken according to the high-level (HL) controller $\qq^H$, and which is translated into low-level or motor action $a_t$ by the low-level (LL) controller $\qq^L$.  We extend the histories $x_t$ and trajectories $\traj$ to appropriately include $z_t$'s. Note that as we elaborate in the appendix this allows for temporally correlated $z_t$'s including the case where $z$ is only sampled once at the beginning of the episode.
% As will be discussed in Section~\ref{sec:related_work}, structuring a policy into HL and LL controllers has been studied e.g.~\cite{heess2016learning,hausman2018learning,haarnoja2018latent,merel2018neural}, but the concept of a default policy has not been widely explored in this context. We discuss the differences between these works and ours in detail in Appendix \ref{appendix:general_framework}.

% In case $z_t$'s can take on many values or are continuous, the objective \eqref{eq:objective:generic} becomes intractable as the marginal distributions $\qq(a_t|x_t)$ and $\pp(a_t|x_t)$ in the KL divergence cannot be computed in closed form. As discussed in more detail in  Appendix~\ref{appendix:general_framework} this problem can be addressed in different ways. For simplicity and concreteness we here assume that the latent variables in $\qp$ and $\pp$ have the same dimension and semantics.
% We can then construct a lower bound for the objective by using the following upper bound for the  KL:
% \begin{align}
% \KL(a_t|s_t)
% \le& \KL(z_t|s_t) + \EE_{\qq(z_t|s_t)}[\KL(a_t|z_t,s_t)],
% \label{eq:kl_upper_bound}
% \end{align}
% which is tractably approximated using Monte Carlo sampling.
% The derivation is in Appendix~\ref{appendix:sub:kl_upper_bound}. 
% Note that:
% \begin{align}
% \KL(z_t|s_t) &= \KL\big(\pi^H(z_t|s_t)\|\pi^H_0(z_t|s_t)\big) \\
% \KL(a_t|z_t,s_t) &= \KL\big(\pi^L(a_t|z_t,s_t)\|\pi^L_0(a_t|z_t, s_t)\big).
% \end{align}
% The resulting lower bound for the objective is:
% \begin{equation}
% \begin{split}
% \textstyle
% \mathcal{L}(\qp, \pp) & \textstyle \geq \textstyle \EE_{\traj}\Big[
% \sum_{t\ge1} \gamma^t r(s_t,a_t)
%     - \alpha\gamma^t\KL(z_t|s_t)\\
%     &\hspace{1.1cm}\textstyle- \alpha\gamma^t\KL(a_t|z_t, s_t)\Big],
% \label{eq:full_objective}
% \end{split}
% \end{equation}
% where $\traj$ is a trajectory that appropriately includes $z_t$'s.

% Finally, it may also be desirable to share some parameters between $\qp$ and $\pp$ which could ensure the latent variables in the shared components have the same semantics. With this in mind, we may consider \bp models with  in the following objective functions: 
% \begin{equation}
% \mathcal{L}(\qp, \pp) & \textstyle \geq \textstyle \EE_{\traj}\Big[
% \sum_{t\ge1} \gamma^t r(s_t,a_t)
%     - \alpha\gamma^t\KL(z_t|s_t)
% \label{eq:shared_objective_LL}
% \\
% \mathcal{L}(\qp, \pp) & \textstyle \geq \textstyle \EE_{\traj}\Big[
% \sum_{t\ge1} \gamma^t r(s_t,a_t) \\
%     &\hspace{1.1cm}\textstyle- \alpha\gamma^t\KL(a_t|z_t,s_t)\Big],
% \label{eq:shared_objective_HL}
% \end{equation}
% This can be seen as imposing a hard constraint setting the KL component to 0. We explore why such formulations may be useful in Section \ref{sec:experiments}.

% For now, we have only formulated a version of our original objective from \ref{eq:objective:generic} with latent variables. There is no guarantee that the policies learnt at the different levels are semantically meaningful or even useful from an RL perspective. However, we can once again turn to the idea of information asymmetry but instead applied across the levels of our structured model. In this case, the latent layer $z$ would then play the role of an \textit{information bottleneck} which forces the higher level to communicate task information of minimal description length in order to control the lower level policy. In this sense, one can thus think of structured models as adding an additional layer with which information regularization can be applied. We study this in greater detail in the following section.

% Structure:
%     % Next, describe hierarchical policies and the variants within that. Discuss how complexity can be either in the HL or LL and since the LL can be transferred directly, we may see an immediate benefit.\label{sec:prob_rl}
% Key points to cover: Theory behind behavioral priors with latent variables. Algorithm to learn with it? 
